SoK: Privacy-Preserving Data Synthesis

As the prevalence of data analysis grows, safeguarding data privacy has become a paramount concern. Consequently, there has been an upsurge in the development of mechanisms aimed at privacy-preserving data analyses. However, these approaches are task-specific; designing algorithms for new tasks is a cumbersome process. As an alternative, one can create synthetic data that is (ideally) devoid of private information. This paper focuses on privacy-preserving data synthesis (PPDS) by providing a comprehensive overview, analysis, and discussion of the field. Specifically, we put forth a master recipe that unifies two prominent strands of research in PPDS: statistical methods and deep learning (DL)-based methods. Under the master recipe, we further dissect the statistical methods into choices of modeling and representation, and investigate the DL-based methods by different generative modeling principles. To consolidate our findings, we provide comprehensive reference tables, distill key takeaways, and identify open problems in the existing literature. In doing so, we aim to answer the following questions: What are the design principles behind different PPDS methods? How can we categorize these methods, and what are the advantages and disadvantages associated with each category? Can we provide guidelines for method selection in different real-world scenarios? We proceed to benchmark several prominent DL-based methods on the task of private image synthesis and conclude that DP-MERF is an all-purpose approach. Finally, upon systematizing the work over the past decade, we identify future directions and call for actions from researchers.

==> app.tex <==

\section{Formal Definition of Neural Network}

\label{sec:formal-nn}

In this project, we consider neural network with ReLU activations, where $\phi(x) = \text{ReLU}(x) = \max\cbr{x, 0}$.
Formally, a ReLU neural network $f: \bbR^{n_0} \to \bbR^{n_y}$ with $L$ hidden layers for classification task is defined as below:

\begin{definition}[Deep Neural Network Model]
	\label{def:nn}
	\begin{equation}
		\left\{
		\begin{aligned}
		x_1 = & \phi(W_0 x_0 + b_0), \\
		x_2 = & \phi(W_1 x_1 + b_1), \\
		\dots, \\
		x_L = & \phi(W_{L-1} x_{L-1} + b_{L-1}), \\
		f(x_0) = y = & W_L x_L + b_L.
		\end{aligned}
		\right.
	\end{equation}
	$n_0, n_1, \dots, n_L$ denote the dimension of $x_0, x_1, \dots, x_L$ respectively.
	$n_{L+1} = n_y$ is the number of classes.
	$W_i \in \bbR^{n_{i+1} \times n_i}, b_i \in \bbR^{n_{i+1}}$.
\end{definition}

Usually for classification tasks, the output is normalized by a softmax layer.
Since softmax layer does not change the relative rank of different dimensions nor the decision, we simply ignore it.

\section{Details of Verification Algorithms}

\label{sec:algo-detail}

In this appendix, we provide the mechanism overview of the verification algorithms in our system, and their implementation details.

\subsection{\ibp~\cite{gowal2018effectiveness}}

\ibp~(interval bound propagation) is based on interval arithmetic.
For the special case of neural networks, let $[l, r]$ denote the input $x$ of $y=Wx+b$.
Then, the output $y$ lies in the interval
$$
	\left[ W_{+} l + W_{-} r + b, W_{+} r + W_{-} l + b \right],
$$
where $W_{+} = \max\cbr{W, 0}, W_{-} = \min\cbr{W, 0}$ are element-wise operators.

Starting from $\left[ x - \epsilon, x + \epsilon \right]$ trimmed by the legal input range, we propagate the interval layer by layer, then we can know the output interval of the final layer, i.e., the confidence score intervals for each class.
If the true class confidence score is always larger than any other wrong classes, we deem the input sample as a robust sample.

\subsection{\fastlin~\cite{weng2018towards}}

In \fastlin, we bound the output of $y = \text{ReLU}(x)$ by a lower line and an upper line.
Suppose the input interval of $x$ is $[l,r]$, if $l<r\le0$, $y=0$; if $0\le l < r$, $y \in [l,r]$; if $l < 0 < r$,
$$
	\dfrac{u}{u-l} x \le \text{ReLU}(x) \le \dfrac{u}{u-l}(x-l).
$$
We symbolically propagate the lower line and the upper line.
Since the composition of lines is still a line, at any time we have linear function for either the lower bound or the upper bound.
Finally, for the last layer, let $y$ denote the true label and $y'$ denote any other labels, we need $f(\cdot)_y \ge f(\cdot)_{y'}$ which in turn means $\left(W_{y:} - W_{y':}\right)x + b_y - b_{y'} \ge 0$, where $x$ is bounded by two linear lines.
Thus, by handling the output intervals of the final two linear functions we obtain a tighter verification approach.

The approach needs the input intervals for all ReLU functions, which are computed recursively by the line bounding technique.
Comparing with the original paper, our implementation computes the common set of both \fastlin~and \ibp~to get the tighter bounds for both $l$ and $u$, thus getting tighter verification results.

\subsection{\directsdp~\cite{raghunathan2018semidefinite}}

In \directsdp, we work on the quadratic form instead of the original form.
Suppose the layer function is $y = \text{ReLU}(Wx)$.
Then we consider the matrix 
$$M = (1 \odot x \odot y) (1 \odot x \odot y)^\T = \left[ \begin{matrix} 1 & x^\T & y^\T \\ x &  xx^\T & xy^\T \\ y & yx^\T & yy^\T \end{matrix} \right] := \left[ \begin{matrix} 1 & x^\T & y^\T \\ x & M_{xx} & M_{xy} \\ y & M_{xy}^\T & M_{yy} \end{matrix} \right]. $$

The constraint is exactly equivalent to
$$
\begin{aligned}
	& y \ge 0, \\
	& y \ge Wx, \\
	& M_{yy} = y \odot (Wx), \\
	& M_{xx} \le (l+u) \odot x - l \odot u.
\end{aligned}
$$

Since $M$ cannot be easily constrained to be the tensor matrix, we only constrain it to be positive semi-definite.
In other words, we eliminate the rank-$1$ constraint for the positive semi-definite matrix $M$.
Then, easily seen, the verification problem is a SDP problem.

In our implementation, we directly extend the constraints to express the activation with bias $y = \text{ReLU}(Wx+b)$.
And our $l$ and $u$, the input interval, is the intersection of both \ibp~and \fastlin.
This input interval is tighter than only \ibp~that is used in the original paper \cite{raghunathan2018semidefinite}.

As mentioned before, we solve the SDP problem using \texttt{SCS} solver.


\subsection{\dualsdp~\cite{fazlyab2019efficient}}

In \dualsdp, we relax the layer constraint to be a set of linear matrix inequality.
Due to the complex forms, we omit them here.
Since linear matrix inequality problem is the dual form of SDP problem, we can still solve it efficiently.
In our implementation, instead of transforming it to be SDP problem, we directly apply conic optimization of \texttt{SCS} solver.

\subsection{\milp~\cite{tjeng2018evaluating}}

In \milp, we express the constraint $y = \text{ReLU}(x)$ by:
$$
	\left(y \le x - l(1-a)\right) \wedge \left(y \ge x\right) \wedge \left( y \le u \cdot a \right) \wedge \left( y \ge 0 \right) \wedge \left( a \in \cbr{0,1} \right).
$$
Then it transforms to a mixed-integer programming problem~(MILP).
There are other MILP constraint forms, but this one is the fastest in practical.

We solve the MILP problem using \texttt{Gurobi} solver, which is exactly the same setting as the original paper~\cite{tjeng2018evaluating}.




==> contents/4.6_additional.tex <==
\subsection{Additional Techniques}
\label{subsec:deep-tech}
\fan{requires work here}
Along a few different dimensions, we introduce the design choices as well as techniques that lead to performance improvement.

\textit{\underline{GAN formulation.}}
The {most common} formulations of GAN include the vanilla GAN~\cite{goodfellow2014explaining,radford2016unsupervised},
% which measures the distribution distance via Jensen-Shannon divergence, 
the Wasserstein GAN~(WGAN)~\cite{arjovsky2017wgan},
% which uses the Wasserstein distance instead, 
and the improved WGAN~\cite{gulrajani2017improved}.
Notably, the theoretical properties of WGAN enables the selection of an optimal clipping threshold for the gradient~\cite{chen2020gs}.
More variants of GAN are summarized in~\Cref{tab:deep}.

\textit{\underline{Privacy accountant.}}
In DP-SGD, the privacy cost accumulates across the training iterations. 
Normally, a privacy accountant is used to track the upper bound of the privacy loss via \textit{adaptive composition} of sequential applications of the Gaussian mechanism.
Research in recent years keep pushing for a tighter bound using different techniques. 
% Proposed by Abadi \etal~\cite{Abadi2016DeepLW} along with the DP-SGD algorithm, the moments accountant derives the bound from the moments.
% The moments accountant~\cite{Abadi2016DeepLW} derives the bound from the moments of the privacy loss.
The moments accountant~\cite{Abadi2016DeepLW} tracks the privacy loss by \textit{adaptive composition} of sequentially applied Gaussian mechanisms and derives the bound of the privacy loss via moments bound.
% , where the moments bound is leveraged to derive an associated upper bound of the privacy loss. 
R\'enyi DP~(RDP)~\cite{mironov2017renyi} builds upon R\'enyi divergence~\cite{renyi1961measures} and supports a tighter privacy analysis;
its appearance boosts the transition to RDP accountant in more recent works~\cite{torkzadehmahani2019dp,chen2020gs,schwabedal2020differentially,kossen2022toward}.


\textit{\underline{Training techniques.}}
GAN is notoriously difficult to train~\cite{salimans2016improved,gulrajani2017improved}.
% DP-SGD further increases the learning instability~\cite{takagi2021p3gm,wang2020dp}, causes additional computational overhead~\cite{xxx}, and leads to performance degradation compared to SGD~\cite{xxx}.
DP-SGD further increases the instability of training~\cite{takagi2021p3gm,wang2020dp}.
Thus, researchers have brought up various techniques %need to be applied 
to facilitate the training procedure. 
% We recall two important steps in DP-SGD: clipping and noise injection. 
To determine a suitable clipping threshold on the gradient norm,
\textit{adaptive clipping} computes a proxy threshold w.r.t. a public dataset~\cite{zhang2018differentially,xu2019ganobfuscator};
\textit{clipping decay} exploits the fact that early stages of training can accommodate more noise~\cite{frigerio2019differentially};
\textit{private norm estimation} obtains the private gradient norms of all samples in a batch and then calculates a DP approximation of their average to use as the clipping norm~\cite{acs2018differentially};
\textit{optimal clipping threshold} can be derived as the approximate upper bound of the gradient norm for certain algorithms~\cite{chen2020gs,zhang2021differentially}.
% dp-GAN~\cite{zhang2018differentially} and GANobfuscator~\cite{xu2019ganobfuscator} propose the adaptive clipping strategy which computes a proxy threshold w.r.t. a public dataset;
% % eliminating the need for a public dataset,
% Frigerio \etal~\cite{frigerio2019differentially} perform clipping decay given that early stages of training can accommodate more noise;
% % much more noise than later stages;
% % a larger amount of noise while less noise can be tolerated in later stages;
% GS-WGAN~\cite{chen2020gs} and Priv-GAN~\cite{zhang2021differentially} derive an approximated upper bound of the gradient norm through the theoretical property of the algorithms.
% of the improved GAN~\cite{gulrajani2017improved}.
% DP-CGAN~\cite{torkzadehmahani2019dp} clip the gradients on real and fake data separately before summing them up and injecting the noise. (i don't understand the benefit of this algorithm)
To decide the scale of the Gaussian noise, 
\textit{noise decay}~\cite{yang2020differential} is proposed  following the similar intuition as that for \textit{clipping decay}.
% Yang \etal~\cite{yang2020differential} propose a noise decay strategy following 
% % the same intuition explained above.
% the aforementioned intuition.
To enable more fine-grained clipping and noise injection, 
stratified clipping is performed over various clustered groups of weights~\cite{zhang2018differentially,wang2020part}.
% parameter grouping is proposed to cluster the weights and perform stratified clipping over different groups~\cite{zhang2018differentially,wang2020part}.
Moreover, %several works find a public dataset helpful in different aspects,
a public dataset is found helpful in several aspects,
\eg, estimating a proxy clipping threshold~\cite{zhang2018differentially,xu2019ganobfuscator} and noise scale~\cite{yu2019differentially},
% serving as a proxy for computing the appropriate clipping threshold~\cite{zhang2018differentially,xu2019ganobfuscator} and noise scale~\cite{yu2019differentially}, 
warm starting~\cite{zhang2018differentially,yang2020differential},
% helping with warm starting~\cite{zhang2018differentially,yang2020differential},
providing a pre-trained embedding model~\cite{fan2021dpnet}.
% The list of techniques could go on and on;
% techniques in both the literature of GAN training and DP-SGD optimization can be leveraged whenever proven helpful.
% techniques from both GAN training (in non-privacy contexts) and DP-SGD optimization (in discriminative modeling) can be borrowed whenever proven helpful.
% ---being the combination of DP-SGD and GAN, 

\textit{\underline{Mixture of models.}} 
% a unique category of models (flexible framework, though the framework itself is questionable)
        Using multiple generative models to model different partitions of the data distribution has been demonstrated to enable easier modeling compared to using one model for all, 
        especially on diverse data samples.
        This further implies benefits on privacy---when fewer training epochs are needed, the accumulated privacy cost will be low.
        In light of such intuition,
        DPGM~\citep{acs2018differentially}, DP-SYN~\citep{abay2018privacy}, and DP-VaeGM~\citep{chen2018differentially}
        use DP-SGD to train DP generative models on disjoint partitions of the dataset, where
        % Their algorithms proceed as follows: first separating the training data into multiple partitions, and then training a DP generative model on each data partition via DP-SGD.
        the partition is performed using either the groundtruth labels~\citep{abay2018privacy,chen2018differentially} or unsupervised clustering through private kernel $k$-means~\citep{acs2018differentially}.
        % can be done via leveraging the groundtruth labels~\citep{abay2018privacy,chen2018differentially} or unsupervised clustering through private kernel $k$-means~\citep{acs2018differentially}.
        % In the partitioning step, the groundtruth labels can be leveraged to guide the partitioning in the supervised setting~\citep{abay2018privacy,chen2018differentially}; or the private kernel $k$-means can be leveraged for an unsupervised clustering~\citep{acs2018differentially}.
        % In the training step, t
        AEs, VAEs, and Restricted Boltzmann Machines~(RBMs)~\cite{tieleman2008training,hinton2012practical} have all been adopted in this framework, but there is no literature that adopts GAN.
        % There is a flexible range of options for the generative models, \eg, AEs~\cite{abay2018privacy}, VAEs~\cite{chen2018differentially}, and Restricted Boltzmann Machines~(RBMs)~\cite{tieleman2008training,hinton2012practical}.
        % There is no literature that fits GAN into this framework, for 
        One 
        potential reason is that GANs are more capable of modeling complicated data distributions.
        % compared to VAEs and RBMs.
        Nevertheless, it is of practical interest to see comparisons between the empirical performance of these different lines of methods.


\textit{\underline{Extension to tabular data.}}\fan{needs work here}
GANs were initially developed for image data~\cite{}.
to extend GANs to deal with tabular data,
it is essential that we embed prior knowledge of the
data (e.g., structural or semantic information) in model
architectures or learning algorithms.
% in the context of privacy, similar requirements and additional challenges.

% Different from image data which GAN is primarily designed for, 
% one unique characteristic of tabular data is the categorical attributes or both categorical and numerical attributes (known as the mixed-type data).
% \mirnegg{Should follow the same notation as in Sec 3: categorical and numerical attribute}. 
% one unique characteristic of tabular data is that it may contain discrete categorical data fields or both discrete and continuous fields (known as the mixed-type data). 
% The presence of 
Discrete categorical data presents a challenge for GAN since the gradient for the discrete variable is zero almost everywhere;
% ---the gradient for the discrete variable is zero almost everywhere, rendering it impossible to train the generator via backpropagation.
even the continuous numerical variable are not the same as those in images due to the lack of Gaussian-like property~\cite{xu2019modeling}.
% To tackle the issue of the discrete data, effective solutions such as the Gumbel softmax~\cite{jang2016categorical} have been proposed; 
To tackle these issues,
% yet for mixed-type data, 
major changes have been made to the data representation, the model architecture, and the learning procedure.

%important table; keep
%\input{tables/tab_GAN_utility_privacy}


==> contents/4.6_discussion.tex <==
\subsection{Comparative Analysis of Generative Modeling Principles}

\noindent\textbf{Compatibility with DP.}\quad
% Diverging prevalence in the non-private and private worlds.
% While almost all principles have had certain air 
% % been studied 
% for data synthesis in the non-private setting, certain instantiations have garnered more attention than others (\eg, AEs, GANs, and diffusion models). However, it is worth noting that the superior methods in the non-private context may not sustain the same level of performance when coupled with DP, as observed in the case of minimax training. Conversely, methods that do not stand out in the non-private world can excel in the private domain, as illustrated by feature alignment. 
% This primarily hinges on the degree of compatibility between the modeling principle and DP.
% Typically, methods that feature stable training, one-time privacy consumption, or low dimensional noise space will enjoy better performance when coupled with DP.
While AEs, GANs, and diffusion models are more favorable for data synthesis in the \textit{non-private} setting, it is important to note that 
these models may not sustain the same level of performance when combined with DP.
%Certain generative modeling principles, such as AEs, GANs, and diffusion models, have received significant attention for data synthesis in the non-private setting. \mirnegg{Rephrase to deliver `These methods shine in non-private data synthesis'} However, 
Conversely, methods that do not stand out in the {non-private} context can excel in the {private} domain, as demonstrated by feature alignment (see~\Cref{subsec:eval-conclusion} for details). This performance discrepancy primarily hinges on the compatibility between the modeling principle and DP. Typically, methods featuring stable training, one-time privacy consumption, or low-dimensional noise space \mirnegg{what is `noise space'} exhibit less performance degradation when coupled with DP.

% unstable training
% high dimensionality
% cumulative consumption



% \mirnegg{Add a paragraph/section after Section 4.5 to summarize different modeling principles from a few angles: compatibility with DP as discussed above, implementation of DP-SGD (end-to-end or other fashion), scalability, sample efficiency, etc.}

\noindent\textbf{Scalability.}\quad

\noindent\textbf{Sample Efficiency. \mirnegg{optional}}\quad

\noindent\textbf{Integration of DP-SGD.}\quad

\mirnegg{Modeling strategy: \textit{directly model data distribution} or \textit{learn efficient representation}}



==> contents/4_deep_copy.tex <==
\section{PPDS via DL-based Methods}
\label{sec:deep}
 \vspace{-3mm} 
\looseness=-1


We move on to PPDS via DL-based methods---methods that leverage deep generative modeling techniques to generate synthetic data. This line of work has garnered increasing interest over the past five years.

\looseness=-1
Deep generative models are renowned for their capability and flexibility in handling data of high dimensionality and generating diverse samples of high quality~\cite{kingma2013auto,goodfellow2014generative,ho2020denoising,song2021scorebased}.
Although these models offer some level of privacy protection empirically~\cite{lu2019empirical,li2019evaluating}, their strong representation power \varun{what is representation power?} \fan{what about ``high capacity''?} can lead to the ``memorization'' phenomenon~\cite{arpit2017closer} which makes room for membership inference attacks~\cite{hayes2017logan,hilprecht2019monte,xu2022mace}. Therefore, it is important to incorporate privacy-preserving mechanisms in deep generative models to provide formal 
privacy guarantees.

\mirnegg{Clarification of the `GAN-heavy' phenomenon in the literature.}

\textbf{Master Recipe.}\quad
Privacy-preserving deep generative modeling fits into the master recipe~(\Cref{fig:framework}).
In the deconstruction stage, one learns the generative model from the given training data; 
in the reconstruction stage, one produces synthetic data by feeding random samples into the generative model. The learning procedure is intertwined with perturbation to ensure DP. 

The instantiations of the master recipe for deep methods differ from that for statistical methods in several aspects, due to the differences in their working mechanisms.
Statistical methods need carefully-crafted modeling and representation selection \varun{what is representation selection?}. The produced compact \varun{i would say latent, not compact?} representation is dependent on the data type. In deep methods, modeling is taken care of by the selection of generative modeling approach as well as model architecture (\eg, deep convolutional GANs for image data), while representation selection is taken care of automatically by the learning procedure. Thus, the enforcement of privacy in deep methods is marginally related to the data type, but closely related to the learning algorithm. The complexity of these learning algorithms necessitate advanced privacy mechanisms \varun{what is a privacy mechanism?} and fine-grained privacy analyses.


\looseness=-1
\textbf{Overview.}\quad
We organize the section by different principles of generative modeling, including adversarial training, auto-encoding mechanism, feature alignment, stochastic simulation, and optimal transport (\Crefrange{subsec:deep-at}{subsec:deep-ot}).
For each approach, we begin with a preliminaries and then discuss the core methodologies or considerations regarding achieving DP for it, followed by paper summary and takeaways. We additionally discuss the technique tools that are used for improving either utility or privacy in~\Cref{subsec:deep-tech}.
Compared to prior surveys~\cite{cai2021generative,fan2020survey,liu2022gdp}, our work offers a more complete picture and systematic categorization. \Cref{tab:deep} presents a summary of the methods under different generative modeling approaches, complemented by several other critical aspects.


\fan{where to introduce each dp technique? -- the first time they appeared?}

\fan{see if we can or need to connect to master recipe in each subsection}

\subsection{PPDS based on Adversarial Training}
\label{subsec:deep-at}

\subsubsection{Preliminaries}
Adversarial training involves training two components in opposition to each other in a minimax game \varun{zero sum game}.
A prominent example
in the context of generative modeling is the Generative Adversarial Network (GAN)~\cite{goodfellow2014generative}.
GANs consist of a generator network that produces samples resembling real data, and a discriminator network that distinguishes between generated and real data. The generator tries to fool the discriminator by producing realistic samples, while the discriminator tries to distinguish between generated and real data. 
The minimax game encourages the generator to generate high-quality and diverse samples~\cite{}. \varun{missing citations below}
GANs have revolutionized generative modeling and led to progress in image synthesis~\cite{}, data augmentation~\cite{}, and text generation~\cite{}.

\subsubsection{Core Methodologies and Considerations}
One natural way to make GANs differentially private is to apply DP-SGD~\cite{}, a widely used method for training deep neural networks under differential privacy. 
DP-SGD ensures the privacy of training examples by adding noise to the gradients (commonly referred to as \textit{gradient perturbation}) computed in each gradient descent step, limiting the influence of individual training examples on the model's parameters.
However, applying DP-SGD to GANs is not straightforward as GANs involve two interdependent models. 
Therefore, careful considerations need to be taken to ensure that the privacy guarantee is preserved while the effectiveness of GAN is maintained.

\varun{the transition here is not smooth}
We consider the threat model for the privacy adversary. 
We focus on the \textit{knowledge} of the adversary, concretely, what the adversary can access. 
This is critical in designing differentially private algorithms, as any information accessible to the adversary must be protected. \varun{this part is unclear; discuss with FW? what is a privacy adversary?}
The strongest adversary (as assumed in Abadi \etal~\cite{Abadi2016DeepLW}) can access all information flow (\eg, outputs, gradients) through all training epochs.
A slightly weaker adversary can access only the generator;
this is a reasonable assumption given that only the generator is typically released for public use.
The weakest adversary sees only the synthetic data, which is a practical assumption that aligns well with the real-world scenarios.
We focus on the first two types of adversaries in this review, which have been widely studied in the literature.
\fanm{We leave the discussion of the model-agnostic weakest adversary to xx. (groundhog day)}


\subsubsection{Paper Summary}~\\

\noindent\textbf{Gradient perturbation on discriminator.}\quad
Most existing works are established against the strongest adversary.
We start by introducing one preliminary approach in several concurrent works~\cite{lu2017poster,beaulieu2019privacy,xie2018differentially,liu2019ppgan,zhang2018differentially}.
They apply DP-SGD only to the discriminator, \ie, clipping and perturbing the gradients of the discriminator.
This is sufficient to ensure DP for the entire system at all times as all information flow is made private.
Specifically, only the discriminator touches the private data, and once the discriminator satisfies DP, the generator also satisfies DP due to the post-processing property.
% First of all, only the discriminator touches the private data.
% Once the discriminator satisfies DP, the generator, whose training relies on the signal (\ie, gradients) of the discriminator, automatically satisfies DP due to the post-processing property.
Additionally, applying DP-SGD only to the discriminator avoids introducing excessive noise to the generator, which could disrupt the training.


\looseness=-1
Frigerio \etal~\cite{frigerio2019differentially} adopt the one-hot representation for the categorical variable and adjust the generator output accordingly.
% Frigerio \etal~\cite{frigerio2019differentially} represent the categorical variable via a one-hot vector and adjust the output layer of the generator such that each categorical variable corresponds to several output units.
% each representing one possible value of the variable.
% Thus, learning the categorical variable is transformed into learning the probability distribution over several outcomes.
CTGAN~\cite{xu2019modeling} proposes a new normalization approach for the continuous variable by modeling it via a variational Gaussian mixture model~(VGM)~\cite{bishop2006pattern}.
% CTGAN~\cite{xu2019modeling} additionally models the continuous variable via a variational Gaussian mixture model~(VGM)~\cite{bishop2006pattern} and represents the value by normalizing it w.r.t. the sampled mode.
These adjustments in data representation and model architecture 
enable effective training of GAN and integration of DP-SGD~\cite{frigerio2019differentially,wang2020part,astolfi2021generating}.
% make GAN training and the integration of DP-SGD possible~\cite{frigerio2019differentially,wang2020part,astolfi2021generating}.
% With the adjustment in data representation and model architecture, the GAN training is made possible and the integration of DP-SGD is naturally enabled~\cite{frigerio2019differentially,wang2020part,astolfi2021generating}.
% Xu \etal first fit the variable to a Gaussian mixture, and then encodes the value of the variable by normalizing it w.r.t. the mode sampled according to the probability densities of each mode 
% Another line of work bypass the challenge of coming up an appropriate representation for mixed-type tabular data, by leveraging the auto-encoding mechanism to automatically learn the representation~\cite{lee2020generating,tantipongpipat2021differentially,torfi2022differentially,fan2021dpnet}.
Another line of work leverages the auto-encoding mechanism to automatically learn the representation for mixed-type tabular data and therefore bypasses the challenge of designing one artificially~\cite{lee2020generating,tantipongpipat2021differentially,torfi2022differentially,fan2021dpnet}.
Basically, a GAN is trained to model the latent representation of an AE, which learns the encoding and decoding mechanisms on the given tabular data.
% Basically, this approach first trains an autoencoder which learns the encoding and decoding mechanism given the tabular data;
% then, with the learned representation in the latent layer, a GAN is trained to model the latent representation. 
Decoding the latents generated by GAN thus yields synthetic tabular data.
% Generation of synthetic tabular data is done through decoding the latents generated by GAN.
For this learning procedure, DP-SGD needs to be applied to the training of AE as well.
% , since the embedding space and the decoding module are also required to be private.
The combination of GAN and AE offers advantages over GAN or AE alone;
it empowers GAN to generate discrete data, and enhances the quality of generation compared to VAE~\cite{tantipongpipat2021differentially}.


\iffalse
\vspace{-1mm} 
\textit{\underline{Graph data.}}\quad
\fan{needs work here; could even considering dropping}
There are two main questions in private graph generation: how to generate graphs and what components should be considered as private in a graph.
For the first question, learning to generate graphs can be posed as learning the distribution of graphs in their various formats of representation---adjacency matrix, edge list, and random walk collection. 
For the second, the privacy requirements differ depending on the concrete application scenarios, with two main types being node-DP and edge-DP~(See \Cref{subsec:privacy-require}).

% Graph data are unique in their several formats of representation---adjacency matrix, edge lists, and a collection of random walks.
% Learning to generate graphs can thus be posed as learning the distribution of real graphs in these representation spaces.
NetGAN~\cite{bojchevski2018netgan} learns the distribution of random walks by incorporating the LSTM architecture~\cite{hochreiter1997long} into GAN.
% in both the generator and the discriminator.
Graph variation autoencoder~(GVAE)~\cite{Kipf2016variational} extends VAE to generate the adjacency matrix 
using an encoder based on graph convolutional network~(GCN)~\cite{welling2016semi}.
% and an inner product based decoder.
% by using a graph convolutional network~(GCN)~\cite{welling2016semi} based encoder as well as an inner product based decoder.
NetGAN and GVAE are used as the generation backbone in the context of private graph generation.
% In private graph generation, these networks serve as the generation backbone;
% different variants of DP (node-DP and edge-DP) are considered according to \textcolor{red}{people's different notions} and the pursuit of privacy in the graph context.
% Given the existence of the intermediate representation, generating a private graph can be achieved by either learning a private representation or building a private graph model from the representation space (\eg, random walks) to graph space.
% In this part, we focus on the former where DP-SGD are leveraged for private learning, and we consider different variants of DP (node-DP and edge-DP) necessitated by people's different notion and pursuit of privacy in the graph context.
Priv-GAN~\cite{zhang2021differentially} and DP-NetGAN~\cite{zheng2022network} applies DP training on the LSTM discriminator of NetGAN.
The former replaces the optimization algorithm by SGLD~\cite{raginsky2017non} and 
achieves node-DP;
% derives the guarantee w.r.t. the change of one node, achieving node-DP; 
the latter uses sets of edges rather than random walks as the input, guaranteeing edge-DP.
DPGGAN~\cite{yang2020secure} adopts GVAE as the generation backbone and further positions it in a VAE-GAN framework~\cite{larsen2016autoencoding} to enforce the global structural fidelity of the generated graph.
They apply DP-SGD in the training of GVAE as well as the VAE-GAN discriminator, and derive the edge-DP guarantee.

We comment that, for the task of DP graph synthesis, a transition took place around 2018, where statistical methods began to fade while deep methods rose to the attention given their capability in handling sequential data and modeling complicated interactions. 
Future work may continue to wire DP mechanisms into other powerful graph generative models~(\eg, GraphRNN~\cite{you2018graphrnn}).
But one core question to always reflect on is whether the achieved privacy guarantee suits the practical need, and, based on that, whether it is possible to devise privacy mechanisms that specifically cater to the graph structure and the desired privacy notion.

\fi

\noindent\textbf{Perturbation on discriminator's signal.}\quad
In the case where only the generator is accessible to the adversary, 
it suffices to build a \textit{privacy barrier} between the discriminator and the generator.
Concretely, 
the training of the generator relies on the signal from the discriminator; 
perturbing the signal could give the privacy guarantee for the generator.
Different works focus on different types of signal and different approaches of perturbation.

\textit{\underline{Partial gradient sanitization.}}\quad
In standard GANs, the signal from the discriminator is the gradient of the discriminator loss w.r.t. the generated sample. 
GS-WGAN~\cite{chen2020gs} note that the gradient update of the generator can be decomposed into a upstream gradient (from the discriminator) and a local gradient (generated sample to the generator parameter) by chain rule, 
of which only the former contains private information.
They therefore propose to perturb the upstream gradient via Gaussian mechanism.
This sanitizes the generator gradient without excessive distortion;
the more informative gradient updates allows better training quality.

\textit{\underline{Private knowledge aggregation and transfer.}}\quad
In the teacher-student framework~\cite{hinton2015distilling}, the knowledge of the ensemble of teacher models is aggregated and then transferred to the student model.
In GANs, the discriminator is analogous to the teacher, its signal to the generator is analogous to the knowledge, and the generator is analogous to the student.
By privatizing the step of knowledge aggregation and transfer, the privacy barrier is built between the discriminator and the generator, leading to the DP guarantee of the generator.

Literature under this category consider two types of knowledge;
they adopt different architectures and different approaches to aggregate the knowledge.
PATE-GAN~\cite{yoon2018pategan} views the discriminator as a classifier and 
considers the output (true/fake) of the discriminator as the knowledge.
They build on PATE~\cite{papernot2017semi,papernot2018scalable}, a differentially private classification scheme, to privatize the discriminator output.
Concretely, they train multiple teacher discriminators and one student discriminator, 
where the student learns on the noisy labels derived by privately aggregating the teachers' votes.
G-PATE~\cite{long2021gpate} and DataLens~\cite{wang2021datalens} consider the gradient of the discriminator as the knowledge. 
The high dimensional gradients are more informative than the single-number output, and thus aggregating on them will preserve more information and better guide the generator.
The architecture used in these two works consist of an ensemble of teacher discriminators and one student generator.
The two works adopt the architecture of multiple teacher discriminators and one student generator,
where the student generator receives the private gradients derived by privately aggregating the teachers' gradients.
Despite the benefits of high-dimensional gradients being more informative, 
aggregating high-dimensional vectors introduces in significantly more amount of noise.
To circumvent the issue,
G-PATE~\cite{long2021gpate} performs dimensionality reduction on the gradients and aggregates the low-dimensional gradients.
They leverage random projection for dimensionality reduction which incurs no additional privacy cost.
Exploiting gradient sparsity and the efforts on gradient compression in distributed learning~\cite{alistarh2018convergence,wangni2018gradient}, 
DataLens~\cite{wang2021datalens} performs stochastic gradient compression on selective dimensions to reduce the sensitivity, so less noise is required for aggregation. 

\begin{takeaway}[Takeaways]
    \fan{needs work here}
\end{takeaway}






\subsection{PPDS based on Auto-Encoding Mechanism}
\label{subsec:deep-ae}

\subsubsection{Preliminaries}
Auto-encoding mechanism~\cite{} learns a lower-dimensional representation of the data known as the latent space, which captures the essential features of the data in a more compact form. 
To generate new samples, one can sample points from the latent space and decode them back to the original data space. 
However, unstructured latent spaces can lead to nonsensical or unrealistic samples~\cite{}. 
To address this issue, researchers have proposed various methods to impose structure on the latent space, such as by constraining it to follow a normal distribution~\cite{} or by incorporating regularizers~\cite{}. 
Variational autoencoders (VAEs)~\cite{} use a probabilistic approach to learn the latent space, which has the nice property of being structured and continuous. 

\subsubsection{Core Considerations and Paper Summary}
The structure of the latent space in auto-encoding mechanisms is crucial for generating high-quality samples.
Researchers adopt various approaches to impose structure on the latent space.
However, incorporating these approaches must be done with caution as they may induce additional privacy cost. 
Below, we discuss these approaches, with an emphasis on how DP is ensured for the end-to-end learning systems.

\fan{needs work here}

\noindent\textbf{Variational Autoencoders (VAEs)}~\cite{kingma2013auto} impose a Gaussian prior on the latent space and optimize the parameters to minimize reconstruction error and KL divergence, leading to a continuous and smooth structure in the latent space.
Since the training of a VAE is end-to-end, one can apply DP-SGD~\cite{Abadi2016DeepLW} during training to achieve DP for the learned VAE~\cite{acs2018differentially,chen2018differentially}.
The data generated by passing a sampled latent through the DP decoder satisfies DP due to the post-processing property.

\noindent\textbf{Latent Space as a Gaussian Mixture.}\quad
DP-SYN~\cite{abay2018privacy} models the latent distribution of a trained AE as a Gaussian mixture.
They first apply DP-SGD to train the AE, and then apply differentially private Expectation Maximization~(DP-EM)~\cite{park2017dp} to estimate the parameter for the Gaussian mixture.
% to enable sampling and generation.
P3GM~\cite{takagi2021p3gm} replaces the encoder with a fixed dimensionality reduction method DP-PCA~\cite{dwork2014analyze} and learns the embedding space through a Gaussian mixture. 
% uses a fixed dimensionality reduction method DP-PCA~\cite{dwork2014analyze} to perform encoding and learns the embedding space through a Gaussian mixture. 
% The separation of encoding and decoding stages reduces the model expressivity and allows more stable training even when DP-SGD is incorporated.
The reduction in model expressivity allows more stable training even when DP-SGD is incorporated.
% In these two works, the parameter estimation for the Gaussian mixture is achieved by the differentially private Expectation Maximization~(DP-EM) algorithm~\cite{park2017dp}.
% This step needs to satisfy DP as well since it directly accesses the sensitive embedding; this is assisted by the DP-EM algorithm proposed in prior work~\cite{park2017dp}.
% we note that the Gaussian mixture modeling needs to satisfy DP as well; 
% this can be assisted by the DP-EM algorithm~\cite{park2017dp} which performs the parameter estimation algorithm Expectation Maximization~(EM) in a DP manner.

\noindent\textbf{GAN Learned Latent.}\quad
Rather than imposing a prior on the latent distribution, a more automated approach learns the latent distribution via a GAN~\cite{lee2020generating,tantipongpipat2021differentially,torfi2022differentially,fan2021dpnet}.
DP-SGD is applied to the learning of both the AE and the GAN.
% Out of consideration for the training stability, AE is often first pre-trained before using GAN to model its latent~\cite{tantipongpipat2021differentially,torfi2022differentially}.
As introduced in the tabular data part, this approach brings benefits over GAN or AE alone.

\begin{takeaway}[Takeaways]
    VAE is not an active area of research in DP generative modeling potentially because its objective is vulnerable to the noise in DP-SGD~\cite{takagi2021p3gm}.
    But AE is widely used in data sanitization due to the nice interpretability of the latent space~\cite{}. 
    For instance, altering latent attributes associated with sensitive information leads to sanitized output.
\end{takeaway}


% Sampling from the latent space of AE and decoding valid data from the sampled latent is almost impossible since there is no regularization on the latent;
% the often used Gaussian prior of VAE 
% In AE trained by reconstruction loss, since there is no regularization on the latent, it is almost impossible to perform sampling in the learned latent space that can lead to valid samples.
% In VAE, Gaussian distribution is often used as the prior to regularize the latent space, yet its representation power may be limited.


% In this part, focus on AE and VAE.
% the latent representation is very critical for the VAE type of generative models 
% latent modeling for various purposes

% why focus on the latent? -- 

% a. use gaussian mixture to model (2 papers with different focus actually, one is to make training stable, the other is to enable generation for AE),

% b. GAN for latent modeling --  others are for generating discrete data

        

% a. general methods and the direct applications (9+2, any difference?)
% b. based on other customized models 
% [TODO: whether to read about the details of those? RCGAN and TCGAN]
% whether to put them under the same category
% e. using other privacy guarantees
% [TO think: whether to put this category here]

% ---------------------------------------------

% \fanm{@Zhuowen}:
% add the GAN papers here; we can discuss how to merge (if possible)

            \iffalse
            Proposed by Abadi \etal~\cite{Abadi2016DeepLW}, gradient perturbation (a.k.a. DP-SGD) has since become a convenient add-on module for deep models that can bring DP guarantees in an almost automated fashion.
            In short, directly applying DP-SGD to existing generative models suffices to produce a DP solution; with this as a basis, more works investigate how to achieve a better utility-privacy tradeoff by promoting utility via improving the model architecture.
            \fi



\subsection{PPDS based on Feature Alignment}
\label{subsec:deep-fa}

\subsubsection{Preliminaries}
Generative models based on feature alignment aim to learn a mapping from a noise distribution to the data distribution by aligning the learned features of the generated data with those of the real data, typically using feature-level distances or similarities.
This approach is particularly advantageous for privacy-preserving generation tasks as it ensures that the learned representation is useful for downstream tasks without enforcing similarity in the data space, which can be beneficial for privacy.

\subsubsection{Core Methodology and Paper Summary}
Feature sanitization is commonly used to achieve DP in feature alignment based generation.
It involves sanitizing the features of the real data and aligning the features of the generated data with the sanitized features.
The learned generative model is DP due to the post-processing property.

Works along this line explore various types of features and distance metrics for generative modeling.

\noindent\textbf{Kernel Mean Embeddings~(KMEs)}~\cite{} map a probability distribution to a reproducing kernel Hilbert space~(RKHS)~\cite{} by taking the mean of kernel evaluations. Maximum Mean Distance~(MMD)~\cite{} measures the distance between two probability distributions in the RKHS, providing a way to enforce distributional constraints in generative modeling. To achieve DP, one can add noise to the KME of real data and minimize the MMD between this noisy KME and the KME of generated data~\cite{harder2021dp,vinaroz2022hermite,harder2022differentially}.


Efficient approximation of the KME can be achieved by using an inner product of feature vectors~\cite{}. 
DP-MERF~\cite{harder2021dp} adopts the random Fourier features~(RFFs)~\cite{}.
However, to achieve good approximation quality, a large number of random features need to be used, which translates into a high-dimensional feature vector, resulting in large amount of noise.
DP-HP~\cite{vinaroz2022hermite} bypasses the problem using Hermite polynomial features~(HPFs), which enjoys the property that a small order of features contain significantly more information than RFFs.
In the image domain specifically, perceptual features~(PFs), \ie, the concatenation of activations from all layers of a pre-trained deep convolutional neural network, have seen success in multiple vision tasks~\cite{gatys2016image,johnson2016perceptual} and also generative modeling~\cite{santos2019learning}.
Building on PFs, DP-MEPF~\cite{harder2022differentially} thus generate samples of high visual quality on CIFAR~\cite{} and CelebA~\cite{} under small $\veps$'s such as 1 and 0.2 (stringent privacy budgets).

\noindent\textbf{Characterization Functions.}\quad
One desired property of the feature space is that two distributions are identical if and only if their features are identical.
This ensures that feature space similarity  translates to similarity data space similarity.
The characteristic function~(CF)~\cite{williams1991probability} enjoys this property---it fully characterizes a random variable's distribution using Fourier transform of its probability density function. 
The characterization function distance~(CFD) 
measures distance between two distributions by calculating the squared difference between their CFs, integrated over sampled frequencies~\cite{heathcote1972test}. 
To achieve DP, one adds noise to the CFs of real data (at all sampled frequencies) and minimize the CFD between these noisy CFs and the CFs of the generated data.

Described above is the core idea of PEARL~\cite{liew2022pearl}.
The authors emphasize that it is crucial to choose a good set of frequencies to avoid a false impression of success, \ie, small CFD on substantially different distributions.
They involve an adversarial objective to tackle the issue, where an adversary is introduced to find a frequency distribution that maximizes the empirical CFD in the inner optimization step.






% \subsubsection{Takeaways}


% - comment on the computation efficiency of this method
% - comment on selection of feature



% selection of features
% selection of distance
% way to enforce DP
% one-time perturbation



% Different types of features can have varying influences on the quality of the generated data for downstream tasks. 
% However, in the case where the downstream task is known, it may be possible to select the most suitable type of feature alignment for that specific task.

\begin{takeaway}[Takeaways]
Feature alignment has several benefits: 
\begin{itemize}[leftmargin=*]
    \item One-shot feature sanitization saves the concern of privacy costs accumulating during training.
    \item The objective functions are easy and efficient to compute and optimize. (DP-MERF~\cite{harder2021dp} finishes training within seconds.)
\end{itemize}
We additionally comment that:
\begin{itemize}[leftmargin=*]
    \item One could choose features most suitable for their data.
    \item MMD suffers from the curse of dimensionality~\cite{ramdas2015decreasing}, so feature alignment based on MMD may fail on high-dimensional data.
\end{itemize}
\end{takeaway}
    

% - influence of diff types of features on utility / generation quality
% - but discuss that but different types of features could be suitable for diff downstream tasks, though generic -- in the case where we may know the downstream task, could use the most suitable feature


% 1. one-time noise
% 2. no adversarial formulation (more stable training)

% The chosen representations (random Fourier features and characteristic functions) retain the desired properties for the data synthesis task while maintaining low sensitivity.



\subsection{PPDS based on Stochastic Simulation}
\label{subsec:deep-ss}

\subsubsection{Preliminaries}
Stochastic simulation is a powerful approach for modeling complex systems~\cite{}.
Diffusion models~(DMs)~\cite{} have successfully adopted this approach in generative modeling to model complex, high-dimensional data distributions with high fidelity, showing promising results in image synthesis~\cite{}.

DMs are suitable for privacy-preserving generation due to their sequential nature. 
By breaking the difficult task of data generation into a series of sequential steps, each step becomes less complex than the one-shot synthesis approach used in other generative models. 
This leads to a more smooth and controllable generation process, 
which can better tolerate the distortion arising from the privacy requirements without significantly compromising the utility of the generated data.

\subsubsection{Paper Summary}
We review two types of diffusion models and discuss how they can be made DP.

\noindent\textbf{Score-Based Generative Models~(SGMs)}~\cite{song2019generative,song2020improved} use a neural network to learn the gradient of the log-density of the target distribution, called \textit{score}~\cite{}.
During training, a Noise Conditional Score Network~(NCSN) is learned to estimate the scores of perturbed data distributions.
When using a Gaussian distribution for perturbing,
% (\ie, $\tilde x \sim \mathcal N (x, \sigma^2I)$), 
the score can be analytically computed.
% as $-\nicefrac{(\tilde x-x)}{\sigma^2}$.
During generation, the score function is used to generate data samples following Langevin dynamics~\cite{}, which involves iteratively updating the current sample in the direction of the gradient.

DPGEN~\cite{chen2022dpgen} makes the point that learning DP scores leads to DP synthesized data.
Their approach consists of two steps. 
First, they create a sanitizied dataset containing Gaussian perturbed samples and their private scores.
Then, they train a NCSN on the sanitized dataset.
The scores are privatized through randomized response~(RR)~\cite{warner1965randomized} by letting each perturbed sample point to one of its nearest neighbors with a certain probability that respects DP, instead of pointing to its counterpart.
The score computed w.r.t. the DP selected sample is thus DP, and the post-processing steps (network training, data generation) are all DP.

The error of RR in the first step is typically small for $\veps>1$, and training the network longer in the second step comes only with the benefit of improving the generation quality but at no cost of privacy.
Thus, DPGEN can synthesize perceptually realistic images of high dimensionality (CelebA~\cite{} and LSUN~\cite{} of size $128\times 128 \times 3$ at $\veps=5$).

\noindent\textbf{Stochastic Differential Equations~(Score SDEs)}~\cite{} aim to model the underlying stochastic process that generates the data.
This involves specifying a SDE that defines a continuous-time trajectory of the data points, which is obtained by adding a diffusion term to the score function.
During the generation process, the Score SDEs solve the SDE using numerical methods (\eg, Euler-Maruyama method~\cite{}) to obtain a discretized trajectory of the data points. 
The discretized trajectory is then passed through a denoiser, which is an NN trained to remove the noise added by the diffusion term. 
\fan{revise}

DPDM~\cite{dockhorn2022dpdm} achieves DP through privatizing the denoiser, the learnable component in Score SDEs.
Concretely, they apply DP-SGD~\cite{} when training the denoiser.
The authors note that the denoiser often has low network capacity, and thus it is amenable to DP-SGD where the magnitude of noise grows linearly with the number of model parameters.
They demonstrate state-of-the-art~(SOTA) performance on various benchmarks.

\begin{takeaway}[Takeaways]
DMs are a promising solution for privacy-preserving high-dimensional image generation, thanks to their tolerance to noise in the sequential steps.
However, one needs to be aware of the sample efficiency issues of DMs, which exacerbate further with increased data dimension.
\end{takeaway}




% it is inconvenient to work with discrete data distributions since scores are only defined on continuous distributions.

% sampling efficiency issue

 % since it involves a large number of Langevin-type iterations

% Gaussian assumption in the denoising step, which is justified only for small step sizes.




\subsection{PPDS based on Optimal Transport}
\label{subsec:deep-ot}
\subsubsection{Preliminaries}
Optimal transport--based generative models~\cite{genevay2018learning,salimans2018improving,patrini2020sinkhorn} use the Wasserstein distance~(W-distance)~\cite{} to measure the distance between probability distributions.
The W-distance is then minimized to generate samples from a target distribution. 
Sinkhorn divergence~\cite{} provides a smooth approximation of the W-distance by introducing a regularization term, eliminating the need for using a discriminator to estimate the W-distance as in WGANs~\cite{}.
This allows for more stable and efficient training of generative models, making it more robust to noise addition and suitable for DP.

\subsubsection{Paper Summary}
DP-Sinkhorn~\cite{cao2021dpsinkhorn} minimizes the Sinkhorn divergence between the real and learned distributions in a DP manner, via applying partial gradient sanitization~\cite{chen2020gs} (introduced in~\Cref{subsec:deep-at}).
The authors propose a semi-debiased Sinkhorn loss to control the bias-variance trade-off, 
since existing empirical Sinkhorn losses is either biased~\cite{} or has large variance while debiased~\cite{}.
Corresponding to the semi-debiased loss,
they split the generated data to calculate the self-term loss (between two splits) and the cross-term loss (between one of the split and the real data). 
They then sanitize the gradient of the cross-term loss w.r.t. the split.
DP-Sinkhorn converges stably and excels at covering multiple modes, a benefit of OT.

\begin{takeaway}[Takeaways]
    Optimal transport eliminates the need for adversarial training, and is thus more robust to training instabilities and suitable for privacy-preserving generative modeling.
    However, it is not suitable for high-dimensional data where solving the optimization problem becomes computationally challenging.
\end{takeaway}

\subsection{Additional Techniques}
\label{subsec:deep-tech}
\fan{requires work here}
Along a few different dimensions, we introduce the design choices as well as techniques that lead to performance improvement.

\textit{\underline{GAN formulation.}}
The {most common} formulations of GAN include the vanilla GAN~\cite{goodfellow2014explaining,radford2016unsupervised},
% which measures the distribution distance via Jensen-Shannon divergence, 
the Wasserstein GAN~(WGAN)~\cite{arjovsky2017wgan},
% which uses the Wasserstein distance instead, 
and the improved WGAN~\cite{gulrajani2017improved}.
% which couples the WGAN objective with a gradient-penalty term. 
% The relative comparisons among these formulations are similar to that in the non-private context~\cite{arjovsky2017wgan,gulrajani2017improved}.
% (justify or rewrite), \eg, [TODO: check the previous non-private papers to find some theoretical justification and private papers to find some empirical evidence]
% theoretical guarantee specifically for improved WGAN (can estimate gradient upper bound)~\cite{chen2020gs}
% theoretical gradient upper bound (SGLD)~\cite{zhang2021differentially}.
Notably, the theoretical properties of WGAN enables the selection of an optimal clipping threshold for the gradient~\cite{chen2020gs}.
More variants of GAN are summarized in~\Cref{tab:deep}.
% the same benefit reaped by the optimization algorithm SGLD~\cite{raginsky2017non}.
% the same benefit can be reaped by replacing the optimization algorithm by SGLD~\cite{raginsky2017non}.
% , which comes with a theoretical gradient upper bound~\cite{zhang2021differentially}.
% Furthermore, conditional GANs (CGAN, AC-GAN)~\cite{mirza2014conditional,odena2017conditional} 
% % and auxiliary classifier GAN (AC-GAN)~\cite{odena2017conditional} 
% are adopted to enable conditional generation; conditional tabular GAN~(CTGAN)~\cite{xu2019modeling} and recurrent conditional GAN~(RCGAN)~\cite{esteban2017real} are each leveraged to accommodate tabular data and time-series data. 

% In terms of the choice of GAN, GAN, 
% both GAN, 
% comparison of the performance? TODO: check the papers and find some evidence
% to generate label
% to accomodate other data types,

\iffalse
Vanilla GAN \& DCGAN
WGAN, improved WGAN
CGAN, ACGAN
RCGAN, CTGAN, NetGAN


        -- GAN type:
        GAN~\cite{goodfellow2014generative}: ~\cite{fan2020relational}
        DCGAN~\cite{radford2016unsupervised}: ~\cite{lu2017poster}

        CGAN~\cite{mirza2014conditional}: DP-CGAN~\cite{torkzadehmahani2019dp}
        AC-GAN~\cite{odena2017conditional}: ~\cite{beaulieu2019privacy}

        WGAN~\cite{arjovsky2017wgan}: DPGAN~\cite{xie2018differentially}, ~\cite{fan2020relational}, PPGAN~\cite{liu2019ppgan}, ~\cite{schwabedal2020differentially}, ~\cite{kossen2022toward}
        improved WGAN~\cite{gulrajani2017improved}: dp-GAN~\cite{zhang2018differentially}, ~\cite{frigerio2019differentially}, GANobfuscator~\cite{xu2019ganobfuscator}, ~\cite{yang2020differential}, GS-WGAN~\cite{chen2020gs}, DPNeT~\cite{fan2021dpnet}, ~\cite{triastcyn2020generating}

        RCGAN~\cite{esteban2017real}: RCGAN~\cite{esteban2017real}
        CTGAN~\cite{xu2019modeling}: DP-CTGAN~\cite{astolfi2021generating}, PART-GAN~\cite{wang2020part}

        NetGAN~\cite{bojchevski2018netgan}: Priv-GAN~\cite{zhang2021differentially}, DP-NetGAN~\cite{zheng2022network}
        GVAE~\citep{Kipf2016variational}: DPGGAN~\cite{yang2020secure}
        VAE-GAN~\cite{larsen2016autoencoding}: DPGGAN~\cite{yang2020secure}
\fi

\textit{\underline{Privacy accountant.}}
In DP-SGD, the privacy cost accumulates across the training iterations. 
Normally, a privacy accountant is used to track the upper bound of the privacy loss via \textit{adaptive composition} of sequential applications of the Gaussian mechanism.
Research in recent years keep pushing for a tighter bound using different techniques. 
% Proposed by Abadi \etal~\cite{Abadi2016DeepLW} along with the DP-SGD algorithm, the moments accountant derives the bound from the moments.
% The moments accountant~\cite{Abadi2016DeepLW} derives the bound from the moments of the privacy loss.
The moments accountant~\cite{Abadi2016DeepLW} tracks the privacy loss by \textit{adaptive composition} of sequentially applied Gaussian mechanisms and derives the bound of the privacy loss via moments bound.
% , where the moments bound is leveraged to derive an associated upper bound of the privacy loss. 
R\'enyi DP~(RDP)~\cite{mironov2017renyi} builds upon R\'enyi divergence~\cite{renyi1961measures} and supports a tighter privacy analysis;
its appearance boosts the transition to RDP accountant in more recent works~\cite{torkzadehmahani2019dp,chen2020gs,schwabedal2020differentially,kossen2022toward}.
% Imposing an assumption on the data distribution, 
% Triastcyn and Faltings~\cite{triastcyn2020bayesian} define the Bayesian DP~(BDP) which is a relaxation of DP, and propose a corresponding BDP accountant.
% Building upon Renyi divergence, Renyi DP~(RDP)~\cite{mironov2017renyi} supports a tighter analysis than the moments accountant.
% This boosts the trend of transitioning to using RDP accountant in more recent works~\cite{torkzadehmahani2019dp,chen2020gs,schwabedal2020differentially,kossen2022toward}.
% , which has been observed in generative models as well~\cite{torkzadehmahani2019dp,chen2020gs,schwabedal2020differentially,kossen2022toward}.

\iffalse
        -- accountant:
        standard composition~\cite{dwork2009differential}: Priv-GAN~\cite{zhang2021differentially}
        moments accountant~\cite{Abadi2016DeepLW}: ~\cite{lu2017poster,beaulieu2019privacy,esteban2017real,xie2018differentially,fan2020relational,liu2019ppgan,zhang2018differentially,frigerio2019differentially,xu2019ganobfuscator,yang2020differential,fan2021dpnet,zheng2022network,wang2020part,yang2020secure}
        RDP~\cite{mironov2017renyi}: ~\cite{torkzadehmahani2019dp,chen2020gs,kossen2022toward,schwabedal2020differentially}
        Bayesian accountant~\cite{triastcyn2020generating}
\fi


\textit{\underline{Training techniques.}}
GAN is notoriously difficult to train~\cite{salimans2016improved,gulrajani2017improved}.
% DP-SGD further increases the learning instability~\cite{takagi2021p3gm,wang2020dp}, causes additional computational overhead~\cite{xxx}, and leads to performance degradation compared to SGD~\cite{xxx}.
DP-SGD further increases the instability of training~\cite{takagi2021p3gm,wang2020dp}.
Thus, researchers have brought up various techniques %need to be applied 
to facilitate the training procedure. 
% We recall two important steps in DP-SGD: clipping and noise injection. 
To determine a suitable clipping threshold on the gradient norm,
\textit{adaptive clipping} computes a proxy threshold w.r.t. a public dataset~\cite{zhang2018differentially,xu2019ganobfuscator};
\textit{clipping decay} exploits the fact that early stages of training can accommodate more noise~\cite{frigerio2019differentially};
\textit{private norm estimation} obtains the private gradient norms of all samples in a batch and then calculates a DP approximation of their average to use as the clipping norm~\cite{acs2018differentially};
\textit{optimal clipping threshold} can be derived as the approximate upper bound of the gradient norm for certain algorithms~\cite{chen2020gs,zhang2021differentially}.
% dp-GAN~\cite{zhang2018differentially} and GANobfuscator~\cite{xu2019ganobfuscator} propose the adaptive clipping strategy which computes a proxy threshold w.r.t. a public dataset;
% % eliminating the need for a public dataset,
% Frigerio \etal~\cite{frigerio2019differentially} perform clipping decay given that early stages of training can accommodate more noise;
% % much more noise than later stages;
% % a larger amount of noise while less noise can be tolerated in later stages;
% GS-WGAN~\cite{chen2020gs} and Priv-GAN~\cite{zhang2021differentially} derive an approximated upper bound of the gradient norm through the theoretical property of the algorithms.
% of the improved GAN~\cite{gulrajani2017improved}.
% DP-CGAN~\cite{torkzadehmahani2019dp} clip the gradients on real and fake data separately before summing them up and injecting the noise. (i don't understand the benefit of this algorithm)
To decide the scale of the Gaussian noise, 
\textit{noise decay}~\cite{yang2020differential} is proposed  following the similar intuition as that for \textit{clipping decay}.
% Yang \etal~\cite{yang2020differential} propose a noise decay strategy following 
% % the same intuition explained above.
% the aforementioned intuition.
To enable more fine-grained clipping and noise injection, 
stratified clipping is performed over various clustered groups of weights~\cite{zhang2018differentially,wang2020part}.
% parameter grouping is proposed to cluster the weights and perform stratified clipping over different groups~\cite{zhang2018differentially,wang2020part}.
Moreover, %several works find a public dataset helpful in different aspects,
a public dataset is found helpful in several aspects,
\eg, estimating a proxy clipping threshold~\cite{zhang2018differentially,xu2019ganobfuscator} and noise scale~\cite{yu2019differentially},
% serving as a proxy for computing the appropriate clipping threshold~\cite{zhang2018differentially,xu2019ganobfuscator} and noise scale~\cite{yu2019differentially}, 
warm starting~\cite{zhang2018differentially,yang2020differential},
% helping with warm starting~\cite{zhang2018differentially,yang2020differential},
providing a pre-trained embedding model~\cite{fan2021dpnet}.
% The list of techniques could go on and on;
% techniques in both the literature of GAN training and DP-SGD optimization can be leveraged whenever proven helpful.
% techniques from both GAN training (in non-privacy contexts) and DP-SGD optimization (in discriminative modeling) can be borrowed whenever proven helpful.
% ---being the combination of DP-SGD and GAN, 

\textit{\underline{Mixture of models.}} 
% a unique category of models (flexible framework, though the framework itself is questionable)
        Using multiple generative models to model different partitions of the data distribution has been demonstrated to enable easier modeling compared to using one model for all, 
        especially on diverse data samples.
        This further implies benefits on privacy---when fewer training epochs are needed, the accumulated privacy cost will be low.
        In light of such intuition,
        DPGM~\citep{acs2018differentially}, DP-SYN~\citep{abay2018privacy}, and DP-VaeGM~\citep{chen2018differentially}
        use DP-SGD to train DP generative models on disjoint partitions of the dataset, where
        % Their algorithms proceed as follows: first separating the training data into multiple partitions, and then training a DP generative model on each data partition via DP-SGD.
        the partition is performed using either the groundtruth labels~\citep{abay2018privacy,chen2018differentially} or unsupervised clustering through private kernel $k$-means~\citep{acs2018differentially}.
        % can be done via leveraging the groundtruth labels~\citep{abay2018privacy,chen2018differentially} or unsupervised clustering through private kernel $k$-means~\citep{acs2018differentially}.
        % In the partitioning step, the groundtruth labels can be leveraged to guide the partitioning in the supervised setting~\citep{abay2018privacy,chen2018differentially}; or the private kernel $k$-means can be leveraged for an unsupervised clustering~\citep{acs2018differentially}.
        % In the training step, t
        AEs, VAEs, and Restricted Boltzmann Machines~(RBMs)~\cite{tieleman2008training,hinton2012practical} have all been adopted in this framework, but there is no literature that adopts GAN.
        % There is a flexible range of options for the generative models, \eg, AEs~\cite{abay2018privacy}, VAEs~\cite{chen2018differentially}, and Restricted Boltzmann Machines~(RBMs)~\cite{tieleman2008training,hinton2012practical}.
        % There is no literature that fits GAN into this framework, for 
        One 
        potential reason is that GANs are more capable of modeling complicated data distributions.
        % compared to VAEs and RBMs.
        Nevertheless, it is of practical interest to see comparisons between the empirical performance of these different lines of methods.


\textit{\underline{Extension to tabular data.}}\fan{needs work here}
GANs were initially developed for image data~\cite{}.
to extend GANs to deal with tabular data,
it is essential that we embed prior knowledge of the
data (e.g., structural or semantic information) in model
architectures or learning algorithms.
% in the context of privacy, similar requirements and additional challenges.

% Different from image data which GAN is primarily designed for, 
% one unique characteristic of tabular data is the categorical attributes or both categorical and numerical attributes (known as the mixed-type data).
% \mirnegg{Should follow the same notation as in Sec 3: categorical and numerical attribute}. 
% one unique characteristic of tabular data is that it may contain discrete categorical data fields or both discrete and continuous fields (known as the mixed-type data). 
% The presence of 
Discrete categorical data presents a challenge for GAN since the gradient for the discrete variable is zero almost everywhere;
% ---the gradient for the discrete variable is zero almost everywhere, rendering it impossible to train the generator via backpropagation.
even the continuous numerical variable are not the same as those in images due to the lack of Gaussian-like property~\cite{xu2019modeling}.
% To tackle the issue of the discrete data, effective solutions such as the Gumbel softmax~\cite{jang2016categorical} have been proposed; 
To tackle these issues,
% yet for mixed-type data, 
major changes have been made to the data representation, the model architecture, and the learning procedure.


\iffalse
        -- techniques:
        1.1 clipping: 
        adaptive clipping [dp-GAN~\cite{zhang2018differentially}, GANobfuscator~\cite{xu2019ganobfuscator}],
        clipping decay~\cite{frigerio2019differentially},
        clip gradients on real and fake data separately [DP-CGAN~\cite{torkzadehmahani2019dp}],
        model selection [PART-GAN~\cite{wang2020part}],
        informed by the theoretical estimation: GS-WGAN~\cite{chen2020gs}, Priv-GAN~\cite{zhang2021differentially}
        1.2 noise injection:
        noise decay~\cite{yang2020differential},
        % noise estimation
        1.3 parameter grouping [dp-GAN~\cite{zhang2018differentially}, PART-GAN~\cite{wang2020part}]
        2. use public dataset: 
        clipping norm estimation [dp-GAN~\cite{zhang2018differentially}, GANobfuscator~\cite{xu2019ganobfuscator}],
        warm starting [dp-GAN~\cite{zhang2018differentially}, ~\cite{yang2020differential}],
        % noise scale estimation, 
        pre-trained embedding [DPNeT~\cite{fan2021dpnet}]
        3. theoretical estimation of the threshold given by WGAN: GS-WGAN~\cite{chen2020gs}, Priv-GAN~\cite{zhang2021differentially}
        4. can support federated learning: GS-WGAN, [TODO: check]
        5. sanitize the gradient from discriminator back to generator (under the new assumption): GS-WGAN
        6. mixed type: change arch for the generator (an output for each value of the categorical variable \cite{frigerio2019differentially}), GAN learning the embedding [DPNeT~\cite{fan2021dpnet}], CTGAN~\cite{xu2019modeling}
        7. time series data, sequence data: recurrent GAN~\cite{esteban2017real}, LSTM inside the generator to model streaming data~\cite{frigerio2019differentially}, NetGAN~\cite{bojchevski2018netgan} (and the two papers based on NetGAN),
        PART-GAN~\cite{wang2020part}
        
\fi






% It directly estimates the distance between the two distributions by solving a regularization problem~\cite{}, which eliminates the need for using a discriminator to estimate the W-distance as in WGANs~\cite{}.


% \input{tables/tab_GAN}

% \input{tables/tab_GAN_metric}
\input{tables/tab_GAN_utility_privacy}

\iffalse
\subsubsection{Preliminaries} \quad
Stochastic gradient descent (SGD)~\cite{massey1951kolmogorov,Kiefer1952StochasticEO} is a standard choice 
for training deep models.
% for optimization  when it comes to training deep models.
% due to its high computational efficiency which is especially desirable for large-scale learning problems~\cite{bottou2010large}.
In each training step, the gradient of the loss 
% on the current batch of training samples w.r.t. the current model parameters 
is computed via backpropagation~\cite{rumelhart1986learning}, and an optimization step is taken along the negative gradient direction to update the model parameters.
% Thus, a natural way to introduce noise into the training procedure is through adding noise to the gradient updates.
Thus, a natural way to enforce DP 
%in the training procedure 
is to perturb the gradients.
Building on this principle, 
Abadi \etal~\cite{Abadi2016DeepLW} propose DP-SGD to train deep models that satisfies DP 
% with only minimum algorithmic changes to SGD.
with minimum changes made upon the vanilla SGD.
Plainly put, DP-SGD adds Gaussian noise with scale proportional to the sensitivity of the \textit{clipped} gradient, and then uses the noisy gradient to update the model.
Due to its convenience and effectiveness, DP-SGD has been widely adopted as an add-on module in many applications~\cite{ziller2021medical,ho2021dpcovid}.
% Yet, incorporating DP-SGD into generative modeling is not as straightforward.
% given the more complicated learning procedure.
% \fanr{In what follows, we xxxx. [TODO: summarize after finishing the parts below]}
\fi


\iffalse
\vspace{-2mm} 
\subsubsection{Paper Summary \mirnegg{change the title}}  \quad
\looseness=-1

% \noindent\textbf{Gradient Perturbation.}\quad

% introduce the works that leverage DP-SGD in generative modeling for different data types and using various techniques to facilitate learning.


%%%%% outline:
% deep models mainly trained by gradient descent;
% adding noise to gradients per training iteration is one natural way to induce noise into the training procedure;
% one previous work DP-SGD has been proposed that can train deep model with DP, and has been widely adopted in training all kinds of deep models (a convenient add-on module);
% DP-SGD clip gradient, add Gaussian noise; use moment accountant;
% DP-SGD adopted in generative modeling as well;
% mostly apply DP-SGD to existing generative models (that handle different data types); mostly only apply DP-SGD to the discriminator;
% on top of this, some works investigate novel methods that improve utility


\looseness=-1
\noindent\textbf{Design Choices and Special Techniques.}\quad

% for improving performance or catering to specific requirements.
% that either lead to performance improvement or cater to specific requirements.

\looseness=-1

\looseness=-1


% on GAN

% on VAE (on AE?)

% on language models?

% other deep models?


\iffalse
\noindent\textbf{{Application on Different Data Types.}}\quad
Mainstream deep generative models were designed for image data at the outset~\cite{kingma2013auto,goodfellow2014generative}.
Despite the universal principle of generation, naively applying the solution for image data to other data types without taking into account their unique characteristics might result in degraded generation performance.
% the concrete instantiations on different data types vary and face different challenges.
% The challenges arise from the unique characteristics of data, which unfortunately cannot be all captured by one plain solution (for image data).
% The challenges arise from the unique characteristics of data.
% The plain solution for image data fails to capture all these characteristics, 
% and it is simply impractical for one solution 
% and overlooking them at all will lead to degraded generation performance.
% To combat oversight of critical structural or semantic information, 
It is therefore essential that we embed prior knowledge of the data (\eg, structural or semantic information) in model architectures or learning algorithms.
In the context of privacy, the generation problem inherits similar requirements and confronts additional challenges.
For example, xxx
In what follows, we xxx \mirnegg{TODO}

\fi

% why generating different types of data is particularly hard in the context of deep generative models, and what is the general philosophy of performing various generations (to me, an ideal solution should try to couple the characteristics, i.e., prior knowledge of data into the architectural and algorithmic design).

% Generation of different data types faces different challenges.
% Privacy-preserving generation inherits the same sets of problems and confronts additional difficulties.


% tabular data is a unique data type which may consist of discrete data and continuous data in different fields of the table.


% introduce tabular data, in which aspect are they unique
% mixed type (discrete data, continuous data)

% discrete data (TSCD): change arch for the generator (an output for each value of the categorical variable \cite{frigerio2019differentially})

% mixed type data (3 previous + 1 DPNeT based): GAN learning the embedding [DPNeT~\cite{fan2021dpnet}], 

% CTGAN time-series data (2)


% \fan{need to add time-series data?}
% 7. time series data, sequence data: recurrent GAN~\cite{esteban2017real}, LSTM inside the generator to model streaming data~\cite{frigerio2019differentially}, NetGAN~\cite{bojchevski2018netgan} (and the two papers based on NetGAN),
% PART-GAN~\cite{wang2020part}
        

% unique in the ways of representation
%     random walks, edges, adjacency matrix
% unique in the different notions of DP
%     node-DP, edge-DP
%     why do each work explicitly focus on one but not the others? (any discussion?)


% (2 NetGAN based + 1 previous)

% Priv-GAN~\cite{zhang2021differentially}, DP-NetGAN~\cite{zheng2022network}, 


% ~\cite{yang2020secure}: GVAE based


% is it possible to apply DP to GraphRNN~\cite{you2018graphrnn}, another popular method for graph generation?



        % naive AE + DP-SGD
        
        % AE with improved architecture + DP-SGD (examples of improved arch: latent, partition-based)

        % \chulin{@zhuowen, try to add transitional sentences between different methods in this paragraph, such as pointing out the limitations of previous works}
        
        \iffalse
        paper list:
        
        general methods: ~\cite{lu2017poster,beaulieu2019privacy}, DPGAN~\cite{xie2018differentially}, 
        PPGAN~\cite{liu2019ppgan},
        dp-GAN~\cite{zhang2018differentially},
        ~\cite{schwabedal2020differentially},
        GANobfuscator~\cite{xu2019ganobfuscator},
        dp-WGAN~\cite{yang2020differential},
        GS-WGAN~\cite{chen2020gs},
        
        direct application of general methods: 
        relational data: ~\cite{fan2020relational},
        medical image data: ~\cite{kossen2022toward}
        
        conditional GAN: DP-CGAN~\cite{torkzadehmahani2019dp}
        
        -- architecture change to accommodate different data types:
        continuous, categorical, and time-series: ~\cite{frigerio2019differentially},
        medical time series (RCGAN): ~\cite{esteban2017real},
        tabular data: DP-CTGAN~\cite{astolfi2021generating},
        time-series data: PART-GAN~\cite{wang2020part}

        -- different priacy guarantees:
        Local DP~\cite{ha2020investigating},
        bayesian DP: ~\cite{triastcyn2020generating}
        
        -- graphs: 
        Priv-GAN~\cite{zhang2021differentially} (node-DP), DP-NetGAN~\cite{zheng2022network} (edge-DP),
        DPGGAN~\cite{yang2020secure} (edge-DP)
        
        
        ---------------------------------------
        
        \fi
        
        
        
        
%         \fanr{-- evaluation
%         membership inference: GANobfuscator~\cite{xu2019ganobfuscator}, ~\cite{frigerio2019differentially} [TODO: check more]
% }        
        
\vspace{-3mm} 
\subsubsection{Takeaways and Open Problems}\quad
We summarize the key takeaway in this subsection:
\begin{itemize}[leftmargin=*]
 \item \textbf{Combination of existing solutions.}\quad
    Many solutions and techniques covered in this subsection are 
    a combination of DP-SGD {and} generative modeling, and their primitive versions typically originate from one of these domains.
    % many solutions and techniques covered above 
    For example, the elegant design of latent modeling via GAN to address the mixed-type tabular data has been proposed in the non-DP generation context~\cite{choi2017generating,sun2021generating,lee2021invertible};
    the technique of using public datasets to facilitate DP-SGD training has been leveraged in the classification setting~\cite{yu2019differentially}.
    PPDS can thus take advantage from the development of both domains~\cite{ho2020denoising,de2022unlocking}.
    
    % Many solutions covered above are built upon their counterparts in the non-DP data synthesis context. 
    % For example, the elegant design of latent modeling via GAN to deal with the mixed-type tubular data has also been proposed in the 
    
    % Being the combination of DP-SGD and GAN, 
    % For example
    % extending approaches (suitable for certain data types, \eg, latent modeling~\cite{choi2017generating,sun2021generating,lee2021invertible}) and techniques (facilitating training, \eg, using public dataset~\cite{yu2019differentially}) in the non-privacy context.
    % realisticity of the assumption --- public dataset (check out PATE-GAN)

% \item \textbf{Improving DP-SGD for better privacy and utility.}\quad
  %  The role of DP-SGD in the methods above is like an add-on module, consisting of several configurable components, \eg, the privacy accountant, the optimization algorithm. Advancements on any of the components (\eg, the RDP accountant~\cite{mironov2017renyi} and the SGLD optimization~\cite{raginsky2017non}) will lead to improvement on privacy or utility \textit{without} sacrificing the other. These individual progress as well as overall shifted efforts (\eg, reducing dimensionality of the gradient updates~\cite{yu2021do,yu2021large}) can be conveniently updated into existing methods to yield better performance.
    
    
    % and end up improving the general approaches.
    
    % DP-SGD serves as an add-on module to the methods introduced above, causi
    
    % can be conveniently incorporated into 
    % add-on module, composed of several modules, 
    % (privacy accountant, optimization algorithm)
    % as a whole, Gradient Embedding Perturbation~(GEP)~\cite{yu2021do}
    
    
    % \item \textbf{takeaways on graph data}
 \end{itemize}   

We also identify an open problem for future research:

\begin{itemize}[leftmargin=*]
    % \item \looseness=-1\textbf{Properties favorable for DP and fundamental changes catering to DP.}\quad
    \item \looseness=-1\textbf{Exploring model/algorithm resilience to DP.}\quad
    DP-SGD is often used in a plug-and-play manner and can be incorporated into the training of almost any deep model. However, it is unclear whether some models or learning algorithms are inherently more robust to noise than others. Identifying the common properties of superior models or algorithms will facilitate the design of new powerful ones that are more resistant to DP.
    % and whether these superior models/algorithms would share any properties. We believe 
    % But will some models or learning algorithms be more robust to noise than others? If so, what are the shared properties among these superior models/algorithms?
    % Benchmarks for validating the intuitions and hypotheses are desirable. Furthermore, based on the discoveries, is it possible to introduce some fundamental changes to the model or learning algorithm that will lead to more resistance to noise and thus better performance under DP?
    
    % Despite its convenience to be incorporated into the training of almost any deep model, we wonder whether some model or learning algorithm will be more robust to noise than others and what are the shared properties among these superior models/algorithms.
    % Benchmarks for validating the intuitions and hypotheses are desirable.
    
    % \item \textbf{Fundamental changes catering to DP.} \quad
    % DP-SGD is often used in a plug-and-play manner. 
    % But we wonder whether it is possible to introduce some fundamental changes to the model or learning algorithm that will lead to more resistance to noise and thus better performance under DP.
    
    % which non-private solution can accommodate noise better? (intuition + benchmark) can we introduce fundamental structural change to the algorithm that specifically accommodate noise better? (e.g., gradient compression in DataLens)
    % \item scalability and performance issue of DP-SGD; application to large models eg language models?
\end{itemize}

\fi

% \fanr{latent modeling:

% -- TODO: discuss the similar tricks in the non-privacy context;
% any comparison between the non-private and private?

% TODO: check GAN survey in the non-privacy context

% (see which tricks have already been used in privacy context and which have not
% any difference in which can accommodate privacy better?)

% structure improvement not invented in the non-privacy context, but works with privacy better? (e.g., the gradient compression in DataLens)

% (is it possible to deal with the problem xxx under the xxx framework?
% }


        
            % \looseness=-1

            % For gradient perturbation during neural network training, we highlight DP-SGD~\cite{Abadi2016DeepLW} (see~\Cref{subsec:gan-prelim}).
            % Following DP-SGD~\cite{Abadi2016DeepLW}, 
            % Liu \etal~\cite{liu2019differentially} incorporate DP-SGD into a single hidden layer AE that synthesizes the user-item rating matrix.
            
            \iffalse
            
            Yang \etal~\citep{yang2020secure} employ DP-SGD in training Graph Variational AE~(GVAE)~\citep{Kipf2016variational}.
            Since GVAE is a graph generative model based on link reconstruction, 
            the synthesized graphs automatically satisfy edge-DP.
            % enforcing DP on it automatically leads to edge-DP.
            Next, we introduce works that improve over vanilla AEs.
            
            
            % For the single hidden layer AE, Liu \etal~\cite{liu2019differentially} compute the \textit{exact} gradient update for model parameters and
            % followed DP-SGD to perform gradient clipping and noise injection at each gradient update step.
            % % achieves the DP AutoRec~\cite{sedhain2015autorec}; 
            % On \textbf{graph data}, 
            % Yang \etal~\citep{yang2020secure} employ DP-SGD for training Graph Variational AE~(GVAE)~\citep{Kipf2016variational}.
            % Since GVAE is a graph generative model based on link reconstruction, enforcing DP on it automatically leads to edge-DP.
            % % , and obtained generated graphs that fulfill edge-DP.
            
            \iffalse
            % Abadi \etal~\citep{Abadi2016DeepLW} provide DP guarantees to the training procedure
            % % and the trained model 
            % by introducing noise in each update of the model parameters during training.
            % The proposed method is named as DP-SGD.
            % Concretely, we add noise to the gradient to induce noisy updates of the model parameters, where the noise magnitude is proportional to the clipped gradient norm. 
            For a single hidden layer AE in the form of AutoRec~\cite{sedhain2015autorec},
            % which uses MSE plus a regularizer as the loss function, 
            Liu \etal~\cite{liu2019differentially} compute the \textit{exact} gradient update for each model parameter, and follow the same idea as DP-SGD~\cite{Abadi2016DeepLW} to perform gradient clipping and Gaussian noise injection at each gradient update step.
            % In this way, they guarantee that the training procedure is differentially private, and therefore the derived model is also DP.
            For the \textbf{graph data} type, 
            Yang \etal~\citep{yang2020secure} proposess to apply DP-SGD~\citep{Abadi2016DeepLW} on the standard architecture of a Graph Variational AE~(GVAE)~\citep{Kipf2016variational} to train a differentially private GVAE (DPGVAE) to generate a graph that achieves edge-DP.
            % leveraging the standard architecture of a Graph Variational AE (GVAE)~\citep{Kipf2016variational} and the standard DP-SGD mechanism~\citep{Abadi2016DeepLW} to train a deep model, 
            % DPGGAN~\citep{yang2020secure} proposes to combine the two to train a differentially private GVAE to reconstruct a graph that achieves edge-DP.
            % Furthermore, to preserve the global structural similarity of the reconstructed graph, DPGGAN~\citep{yang2020secure} leverages a structural-oriented graph discriminator based on GCN and the framework of VAEGAN~\citep{gu2018dialogwae}.
            \fi
            
            \noindent \textit{2. DP-SGD on AE with Latent Modeling.}\quad

        latent modeling 
        -- mixed-type data (learning embedding): 
        network traffic: DPNeT~\cite{fan2021dpnet} 
        [TODO: for this type of learning latent with GAN, check where noise is applied --- should be discriminator and decoder]

            
            Both AE and VAE have certain limitations that hinder their performance in terms of the ability or quality of generation.
            Since the latent of AE is not regularized, it is almost impossible to generate valid samples via sampling from the latent space and passing the sampled latent to the decoder. 
            This limits the usage of AE as a generative model that can synthesize infinite number of samples.
            Although the limitation is addressed in VAE by imposing regularization on its latent space, the generation quality of VAE is unsatisfying due to the limited representation power of the Gaussian latent and the constrained form of the loss function. 

            % Comparatively, VAE is equipped with the generative capability thanks to the regularization on its latent space. 
            % Yet, the quality of generation 
            
            The aforementioned issues can be tackled or largely alleviated by more advanced and flexible modeling of the latent.
            DP-SYN~\cite{abay2018privacy} models the latent of an AE using a Gaussian mixture and performs the parameter estimation via the Expectation Maximization (EM) algorithm~\cite{moon1996em}.
            For the privacy purpose, aside from adopting DP-SGD in training AE,  
            the step of latent modeling is also implemented in a differentially private manner following the prior work DP-EM~\cite{park2017dp}.
            Similarly, P3GM~\cite{takagi2021p3gm} proposes to model the latent via a Gaussian mixture learned by DP-EM. 
            Adapting upon the vanilla VAE, P3GM encodes the mean variable via the dimensionality reduction algorithm DP-PCA~\cite{dwork2014analyze}, and learns the decoder given the fixed encoder. 
            Although at a cost of weaker expressive power compared with vanilla VAE, P3GM is more tolerant to the noise of DP-SGD  and its training becomes more stable.
            % The motivation of this work is to increase the stability 
            
            Another line of works~\cite{lee2020generating,tantipongpipat2021differentially,torfi2022differentially} model the latent via a GAN. 
            They couple the AE with a GAN where AE is trained for reconstructing data and GAN is trained for generating the latent representation of the AE. 
            After training, the generation of synthetic samples is performed in the following manner: 
            sampling a noise from the prior distribution of GAN, passing the noise through the GAN generator, passing the generated latent representation through the decoder.
            To achieve DP in this pipeline, we only require that DP-SGD be involved in the training of the AE and the GAN discriminator but not the GAN generator, for the obvious reason that the GAN generator does not access the private data.
            % with the following two steps: 
            % the GAN component generates the latent representation from a noise sampled from the prior distribution, and then the decoder takes in the latent representation and generates the synthetic sample.
            Regarding the training approach,
            it is viable to train the GAN and the AE in an alternative manner~\cite{lee2020generating};
            actually, first pre-training the AE and then training the GAN along with the freezed AE~\cite{tantipongpipat2021differentially,torfi2022differentially} would lead to more stable training.
            % Regarding the model architecture, convolutional AE and convolutional GAN are better at handling the correlated features~\cite{torfi2022differentially}, and recurrent AE is more appropriate for sequential data~\cite{lee2020generating}.
            We emphasize that, the combination of GAN and AE offers advantages over AE or GAN alone. 
            GAN allows for the possibility of generating infinite samples, and AE compensates for the incompetency of GAN in generating discrete data distribution such as Electronic Health Record~(EHR)~\cite{lee2020generating,torfi2022differentially}.
            Additionally, it is empirically demonstrated that this combination leads to higher quality of generation compared with VAE~\cite{tantipongpipat2021differentially}.
            % The adversarial fashion of GAN training leads to higher quality of generation, and the involvement of AE compensates for the incompetency of GAN in generating discrete data distribution such as Electronic Health Record~(EHR)~\cite{lee2020generating,torfi2022differentially}.
            
            % data-dependent
            
            
            
            % required to be DP, and this is achieved by leveraging the DP-EM module proposed in a previous work~\cite{park2017dp}.
            
                % AE: enable AE to generate infinite amount of data
                
                % VAE: achieve more flexibility \& representation power on the latent
                
                % generally: improving generation quality (+GAN) and mode coverage (+AE)
                
                % generating mixed-type data / discrete data; pure GANs fail when the data is a mixture of continuous and discrete data 

        
        
        % [model the latent via parameter estimation --- EM / MoG]
        % P3GM~\cite{takagi2021p3gm} --- stability
        % Abay \etal~\cite{abay2018privacy} --- 
        
        % [model the latent via GAN]
        % \cite{lee2020generating,tantipongpipat2021differentially,choi2017generating,torfi2022differentially}
        % When the type of the generated data is complex (\eg, mixed-type data that contains categorical features, binary features, and real-valued features), it is unrealistic to assume the latent representations can be modelled simply by a Gaussian distribution or Gaussian mixtures~\citep{acs2018differentially,abay2018privacy}.
        % % as in DPGM~\citep{acs2018differentially} (or DP-SYN~\citep{abay2018privacy}). 
        % For this complex representation, researchers have resourced to sophisticated models, such as GANs~\citep{goodfellow2014generative}.
        % A practical example for \textit{discrete} tabular data is the work of Choi \etal~\citep{choi2017generating}, who train a GAN to learn the complex distribution of the latent space of a pre-trained AE, which produces a GAN capable of producing privacy-preserving datasets.
        % \begin{comment}
        %   Specifically, for \textit{discrete tabular} data 
        % in Choi \etal~\citep{choi2017generating} and \textit{mixed-type} \textbf{tabular data} in Tantipongpipat \etal~\citep{tantipongpipat2021differentially}, they both train a GAN to learn the complex distribution of the latent space of a pre-trained AE.   
        %         The final generated data obtained by passing the GAN output through the decoder is then private.
        % \end{comment}
        % Improving the privacy guarantees of Choi \etal's approach, and in the context of \textit{mixed-type} tabular data, Tantipongpipat \etal~\citep{tantipongpipat2021differentially} introduces DP in the training of the AE with DP-SGD.   
        
        \iffalse
        \noindent \textit{3. DP-SGD on AE in Mixture of Models.}\quad
        % DPGM~\citep{acs2018differentially}, DP-SYN~\citep{abay2018privacy}, and DP-VaeGM~\citep{chen2018differentially}
        When the data diversity is high, separately modeling different distributions would be more beneficial.
        In terms of model utility, modeling similar data samples will be easier than modeling highly diverse data; thus, the images generated by each model would be of higher quality.
        % especially under DP requirements.
        % Given the intuition of separately modeling the distribution of highly distinctive data is a simpler task than jointly modeling them all, such separated modeling can offer both utility and privacy benefits. From an utility perspective, the image generated by each model would be more plausible; 
        Regarding privacy, since training usually requires fewer iterations, one could reduce the amount of consumed privacy. 
        \begin{comment}
              regarding privacy, since training is easier, the total amount of consumed privacy would be smaller due to potentially reduced training iteration and large magnitude of allowed noise.   
        \end{comment}
            DPGM~\citep{acs2018differentially}, DP-SYN~\citep{abay2018privacy}, and DP-VaeGM~\citep{chen2018differentially} capture this idea and propose to first separate the training data into multiple partitions and then train a DP generative model on each data partition via DP-SGD. 
            Depending on the assumption on the availability of groundtruth labels, the partitioning step is either done via leveraging groundtruth labels~\citep{abay2018privacy,chen2018differentially}) or 
            performing private kernel $k$-means for an unsupervised clustering~\citep{acs2018differentially}.
            % The selection of base generative models on each partition is flexible. Both VAE and AE coupled with an EM module 
            
        \fi
        
        DP-GAN~\cite{xie2018differentially} is the first known work to adapt DP to GANs, which modifies WGAN~\cite{wgan} by adding Gaussian noise to the gradients of the Wasserstein distance loss during training. It uses moments accountant~\cite{Abadi2016DeepLW} to track the privacy cost. dp-GAN~\cite{zhang2018differentially} improves over DP-GAN by incorporating the improved WGAN~\cite{Ishaan2017improved}, adaptive clipping and parameter grouping. Similarly, GANobfuscator~\cite{xu2019ganobfuscator} adopts adaptive clipping and quantitatively evaluates the relationship between privacy budget and information disclosure.
        % DP-GAN can be applied to both structured data such as the tabular dataset Electronic Health Records (EHR), as well as unstructured dataset such as MNIST.
        % Practitioners can apply DP-GAN to both structured and unstructured data.
        dp-GAN-TSCD~\cite{frigerio2019differentially} extends dp-GAN to generate time series (e.g. multivariable table data), where TSCD stands for time
        series, continuous and discrete data.
        DP-CGAN~\cite{torkzadehmahani2019dp} leverages conditional GANs~\cite{cgan} to produce synthetic data and labels simultaneously. It accommodates a new gradient clipping procedure for real and synthetic data separately to reduce privacy budget, and it also leverages the RDP accountant~\cite{mironov2017renyi} to provide a tighter bound for the privacy budget\chulin{"tighter" --- compared to which work?}.
        
        \fi
 \vspace{-2mm} 

 \iffalse 
\subsection{PPDS via Private Knowledge Aggregation and Transfer}
\label{subsec:deep-aggregation}
\vspace{-3mm} 
\subsubsection{Preliminaries} \quad
Knowledge aggregation and transfer has long been studied in the non-private context~\cite{breiman1996bagging}; 
distilling the knowledge learned by an ensemble of models into one single model enables easier deployment~\cite{hinton2015distilling}.
This, when viewed from the privacy perspective, coincides well with 
the constraint on the access of private data and the privacy requirement on the learned model. 
Hamm \etal~\cite{hamm2016learning} provide a solution to transfer the knowledge learned by local classifiers at multiple parties to a global classifier while satisfying DP;
Papernot \etal~\cite{papernot2017semi,papernot2018scalable} propose PATE, a more general framework independent of the learning algorithm of the local teacher classifiers, where the global student classifier learns on public data under the noisy guidance of the teacher classifiers.
Despite the progress and promising results in the classification setting, the generalization to generative modeling still faces several challenges.


\vspace{-3mm} 

% principle? --
% - what to aggregate on?
% more information, better utility, but consumes more privacy budget
% need to design methods to aggregate high-dimensional information, e.g., projection, compression
%     can leverage ideas from dimensionality reduction or distributed training communication
% how does the distributional aggregation bypass the issue?? to check

% design choice
% - how many teachers?
% trade-off 


% PATE-GAN~\cite{yoon2018pategan}
%     SeqPATE~\cite{tian2021seqpate}
% G-PATE~\cite{long2021gpate}
% DataLens~\cite{wang2021datalens}

% essentially, gradient aggregation and distribution aggregation use more information (than the label) to train the model

% unique about the distribution aggregation: public dataset, private dataset
% check other language models?
% (does SeqPATE fall under generation?

% assumption on information accessible by the adversary?

% In PATE-GAN, 
% compared with PATE, no assumption on existence of the public dataset
% discriminator -- 
% teacher discriminators not DP, 
% student discriminator satisfies DP,
% (why train student only on generated samples?)
% generator -- 
% post-processing 

% In GS-WGAN: no aggregation at all, should not be place here

% In G-PATE:
% teacher discriminators
% student generator
% (eliminate the student discriminator in between)
% aggregation: random projection, histogram, PATE aggregation
% [only the generator is accessible by the adversary]

% In DataLens:
% compare with G-PATE, different approach of aggregation
% aggregation: top-k compression, summation and thresholding
% [only the generator is accessible by the adversary]

% In SeqPATE: 
% reduce sequence generation to next word prediction? hmm...
% is the method generalizable to image domain (assuming public dataset)?
% what if we have public dataset in PATE-GAN?

\subsubsection{Takeaways and Open Problems}
\quad We summarize the key takeaway in this subsection:

\begin{itemize}[leftmargin=*]
    \item  \textbf{Two trade-offs.} 
    %via detailed design choices or algorithmic parameters can allow finer control of the trade-off as well as targeted improvement on certain components.
    In the teacher-student framework, we identify a high-level trade-off (in design choice) and a low-level one (in parameter choice).
    The high-level one concerns the form of knowledge to aggregate on and transfer---more informative knowledge leads to more powerful model but 
    costs more privacy budget;
    the low-level one centers around the parameter for the number of teachers---fewer teachers can accommodate less noise yet each one is of relatively good quality. 
    The first trade-off helps the selection of the form of knowledge and subsequently promotes targeted designs to save privacy budget when using that knowledge.
    The second one enables finer control of the trade-off.
    
    
    % \textbf{Trade-off between utility and privacy.}
    % We identify two levels of trade-off under the teacher-student framework in this subsection. 
    % The high-level tradeoff consists in the form of knowledge to aggregation and transfer. 
    % As we have pointed out, aggregation on more informative knowledge leads to more powerful model but 
    % costs more privacy budget due to the high dimensionality of knowledge. 
    % The low-level tradeoff centers around the 
    
    % concretize the utility-privacy tradeoff in concrete design choices/parameters so as to allow better control the tradeoff (\eg, teacher number in teacher-student model) and allow targeted improvement on certain components (\eg, what information to transfer and how to save budget when using that info)


\end{itemize}

We also identify an open problem for future research:
\begin{itemize}[leftmargin=*]
    
\item \textbf{Extension to the federated setting.} \quad
    The teacher-student framework in this subsection is naturally extendable to the federated setting, where each user corresponds to a teacher and the central server corresponds to the student.
    However, there exist specificites of FL that might hinder the direct application of the teacher-student framework, such as clients with non-iid datasets, privacy definitions beyond the standard one (e.g., user-level DP) and constraints on the communication infrastructure. On the other hand, this also implies more opportunities for researchers.
    % But there may exist challenges specific to FL that hinder direct adaptation, such as clients with non-iid datasets, DP definitions beyond the standard one (\eg, user-level DP), constraints on the communication infrastructure.
    % These specificities bring about more challenges and opportunities.
    % \fan{TODO: check advantages of other methods specifically designed for FL generation}
\end{itemize}    
    % % But there are several issues to be alerted of in the adaptation.
    % First, methods here are designed for iid datasets, while the users may be non-iid in FL.
    % Second, methods here are all designed to achieve standard DP, while other DP guarantees such as user-level DP or local DP may be desired in FL.
    % Third, the practicality of these methods needs to be checked against the concrete scenario in FL.
    % constraints on communication bandwidth in FL needs to be checked against these methods.
    
    % additional constraint in the federated setting;
    % non-iid user

% \fanr{TODO: 
% summarize the tradeoff between more utility and more privacy cost;
% discuss the more nuanced trade-off related to the \#teacher;
% details on partitioning and training;
% discuss the public dataset;
% check the distributional aggregation in SeqPATE~\cite{tian2021seqpate} and see whether applicable here;

% which may be suitable for extending to federated learning?
% - GS-WGAN
% - all papers here under the teacher-student framework
% - others?


% 1. what information to choose
% 2. how to save budget using that information

% add discussion on the empirical results
% }

\fi

\iffalse

\fan{TODO: remove objective perturbation part; add an others part and cover post-processing together}



\subsection{PPDS via Objective Perturbation}
\label{subsec:deep-objective}

\bo{gradient perturbation is special case of objective perturbation. not sure the logic here but maybe explain why they are separated and the rational}
\subsubsection{Preliminaries}
Setting aside the optimization algorithms and the randomness during training, 
the objective function determines the solution set of an optimization problem.
Perturbing the objective function to satisfy indistinguishability under the presence/absence of any one sample thus leads to DP guarantee on the solution to the optimization problem, \ie, the learned model.
% If we regard the previous two approaches gradient perturbation and private aggregation as `means', then objective perturbation can be viewed as the `ends'.
% Perturbing the objective function in a way that leads to indistinguishability under the presence/absence of any one sample
% Objective perturbation produces a perturbed objective function
% proposes to solves the optimization problem w.r.t. the perturbed objective function, where the perturbation leads to the indistinguishability under the presence/absence of any one sample.
The first works by Chaudhuri \etal~\cite{chaudhuri2008privacy,chaudhuri2011differentially} 
along this line propose a solution for the convex and twice differentiable objective function.
Generalizing over the above idea and targeting at addressing the convexity limitation,
Zhang \etal~\cite{zhang2012functional} propose the functional mechanism which first represents the objective function in the polynomial form through Taylor expansion and then adds Laplace noise to each coefficient in the expansion.

% \noindent\textbf{Objective Perturbation.}\quad
\subsubsection{Paper Summary}
Applying the functional mechanism on the objective function of the GAN discriminator directly leads to a DP generative model~\cite{zhang2019differentially}.
The major limitation of the functional mechanism is the low-order polynomial form approximation, which is unrealistic for deep neural networks with complicated architectures.
We note that the requirement for the low-order approximation arises from the need of computing a perturbed objective function for the given task, model, and privacy budget beforehand.
One could circumvent the trouble by adding noise to the objective function on the go and tracking the privacy cost via a privacy accountant.
RDP-GAN~\cite{ma2020rdp} adds Gaussian noise to the objective of the GAN discriminator and uses RDP accountant~\cite{mironov2017renyi} to track the privacy loss.
Thanks to the flexibility of privacy accounting, it allows adjusting the noise scale dynamically depending on the model performance.
It is scalable to all existing model architectures and can be integrated conveniently.


% In contrast to these works which compute a preset perturbed objective function via calibrating the noise for the given task and model architecture, 
% another viable approach is to add different amount of noise to the objective function on the go and track the privacy cost via a privacy accountant.

% 1. model architecture
% 2. present - inconvenience




% earliest work: ~\cite{chaudhuri2008privacy,chaudhuri2011differentially}
% convex and twice differentiable loss for a regression task
% add noise to the objective function
% compute minimizer w.r.t. the fixed perturbed objective

% later, functional mechanism: ~\cite{zhang2012functional}
% applicable for a large class of optimization
% add calibrated noise to the coefficient



\iffalse
            Also known as the \textit{functional mechanism} in the context of regression analysis~\citep{zhang2012functional}, this type of method achieves DP by introducing noise to the objective function and performing minimization w.r.t. the perturbed objective. 
            % Furthermore, in order to obtain the objective function with bounded degrees for the purpose of adding bounded noise, Zhang \etal~\citep{zhang2012functional} propose a method for deriving the approximate polynomial form of the objective function building upon Taylor expansions.
            Leveraging this approach, Phan \etal~\cite{phan2016differential} and Ren \etal~\citep{ren2019recommender} achieve DP guarantee for a single hidden layer AE that synthesizes the user-item rating matrix.
            However, the application of objective perturbation is constrained in the sense that the form of the objective function cannot be too complicated, for the sake of sensitivity computation. 
            Thus, more advanced approaches need to be considered for deep models.

\fi

% Also known as the \textit{functional mechanism} in the context of regression analysis~\citep{zhang2012functional},
% \zwc{I commented out the description of functional mechanism here, since it referes to ``In functional mechanism, the objective function f(w) is ﬁrst represented in polynomial forms through Taylor Expansion and then the Laplace noise is injected into the polynomial coefﬁcients of the expansion'' (cited from \cite{zhang2019differentially}). However, RDP-GAN~\cite{ma2020rdp} directly adds noise to the value of the loss function. We can add more details of the functional mechanism if necessary.}



% -- standard objective perturbation (functional mechanism) does xxxx

% limitation of standard objective perturbation

% -- RDP-GAN performs objective perturbation on a per iteration basis

% \fanr{TODO: strengths of this method
% comparison with gradient perturbation
% (other convenient gradient perturbation -- the overbill paper)
% discuss the empirical performance
% }

\subsubsection{Takeaways and Open Problems}

We summarize the takeaway in this subsection:

\fi
% Objective perturbation provides a 


\iffalse
This type of method achieves DP by introducing noise to the objective function and performing minimization w.r.t. the perturbed objective.
Zhang~\etal~\cite{zhang2019differentially} propose PPGAN that perturbs the objective function of discriminator by injecting Laplace noises to the training objective through \textit{functional mechanism}\chulin{cite or explain}. 
RDP-GAN~\cite{ma2020rdp} takes a different approach that directly adds random noise on the value of the loss function and tracks privacy cost with RDP accountant\chulin{cite RDP accountant}.
The authors also propose an adaptive noise tuning algorithm that decreases the magnitude of noise as the training continues.
Both PPGAN and RDP-GAN demonstrate superior performance than the baseline approach DP-GAN~\cite{xie2018differentially} on MNIST, which directly adapts DP-SGD to GANs.
\fi


\iffalse
\vspace{-2mm} 
% \subsection{Pre-Processing and Post-Processing Stage Privacy Preservation}
\subsection{PPDS via Generalized Input Perturbation}
\vspace{-2mm} 

\subsubsection{Preliminaries} \quad
Thanks to the post-processing property of DP, performing perturbation on the algorithm input, once and for all, can lead to DP guarantee on the output (and all downstream tasks).
On the one hand, 
% compared to enforcing privacy at the training stage (\Cref{subsec:deep-gradient,subsec:deep-aggregation}), 
input perturbation circumvents the need for modifying the training algorithms (\Cref{subsec:deep-gradient,subsec:deep-aggregation}) to achieve DP, as well as its subsequent consequences such as training instability or increased computational overhead.
On the other hand, naive input perturbation methods that determine the scale of noise solely based on data regardless of the concrete task will introduce excessive noise and end up impairing the utility.
% Naive input perturbation algorithm such as 
% randomized response~\cite{warner1965randomized,greenberg1969unrelated}
% is straightforward and easy-to-use. 
% Compared to enforcing privacy at training stage (\Cref{subsec:deep-gradient,subsec:deep-aggregation})%,subsec:deep-objective}),  
% , input perturbation, once and for all, leads to DP for all subsequent tasks, circumventing the needs for modifications to the training algorithms (\eg, DP-SGD) that incur instability or increase computational overhead.
% On the other hand, determining the scale of noise solely based on data regardless of the concrete task will introduce excessive noise to data; such severe distortion will end up impair their usability.
In what follows, we go beyond the naive input perturbation and introduce \textit{generalized input perturbation} that alleviates the issues but retains the benefits.




% In \Cref{subsec:deep-gradient,subsec:deep-aggregation,subsec:deep-objective}, we mainly focus on enforcing DP during training stage. 
% pre-processing stage also harbors the possibility for inducing DP, given its post-processing property.
% In fact, 
% naive input perturbation such as 
% randomized response~\cite{warner1965randomized,greenberg1969unrelated}
% is quite straightforward and easy-to-use. 
% However, their simplicity leads to their inferior performance compared with training stage privacy mechanisms.
% Determining the scale of noise solely based on data regardless of the modeling of data in the learning procedure will inevitably introduce excessive noise to data, which eventually impairs the performance.
% \fanr{The nice thing is, xxxxx [pre-processing stage and post-processing stage operations can also be related to the learning algorithm / modeling], to summarize later

% benefit is that the model training can be performed in a non-private manner and incurs no additional privacy cost
% }

% Enforcing DP during training stage is most commonly considered.
% As shown in~\Cref{subsec:deep-train}, multiple elements are involved in training, allowing higher design flexibility.
% Moreover, interweaving the privacy mechanism into the learning algorithm enables more refined privacy analysis and better control over the trade-off between utility and privacy.
% Though not as prominent, 

% pre-processing stage: convenient; once and for all; no issues of DP-SGD (learning instability, computational overhead)


% 1. training stage is one major stage
% multiple elements to consider during the training stage---objective, gradient, information flow in unique arch---allows design flexibility, lots of possibilities;
% privacy mechanism tightly intertwined into the learning algorithm---more refined

% 2. pre-processing and post-processing are feasible, thanks to the post-processing property

% naive input perturbation and output perturbation are two easiest and most straightforward solutions to consider
% input perturbation -- random response?
% output perturbation -- standard laplace mechanism

% training stage techniques are often more advanced than them, since they take into account the training

% pre-processing stage where preliminary processing is applied on data before sending them into the training pipeline, 
% and post-processing stage where 

\vspace{-2mm} 
\subsubsection{Paper Summary}

% input perturbation and output perturbation 

% for pre-processing stage:
% two types of input perturbation
% 1. where the scale of the noise %introduced in input perturbation 
% is determined solely by the input data regardless of the subsequent learning algorithm ---  usually introduces excessive noise that leads to undermined performance.
% Imtiaz~\etal~\cite{imtiaz2021synthetic}

% 2. where the input perturbation is guided by the training procedure
% ~\cite{harder2021dp, liew2022pearl, torkzadehmahani2019dp}
% DP-MERF~\cite{harder2021dp}
% PEARL~\cite{liew2022pearl}
% DPGEN~\cite{chen2022dpgen}


% for post-processing stage:
% Private PGB~\cite{neunhoeffer2021private}

% the scope of papers to cover in this part: 
% \underline{\textit{Method Principle.}}
% 1. an appropriate representation
% 2. a learning algorithm
% \fanr{TODO: need to separate the pre-processing and post-processing stage?}
% *may not need to introduce the detail of this naive paper*
% Imtiaz~\etal~\cite{imtiaz2021synthetic} propose to apply Laplace mechanism on the input data space or output data space, \ie, the sensitive data used for GAN training or the synthetic data produced by a trained GAN.
% Although the model training can be performed in a non-private manner and incurs no additional privacy cost,
% their approach already suffers from the tremendous amount of noise (or the huge privacy loss) during pre-processing or post-processing.

\looseness=-1
Motivated by the poor utility-privacy trade-off obtained by naive input perturbation~\cite{imtiaz2021synthetic},
% Directly performing input perturbation on \textit{data space} and training a generative model on the perturbed input can provide DP guarantee but with poor utility-privacy trade-off~\cite{imtiaz2021synthetic}.
we ask: \textit{is it possible to perform input perturbation better suited to the task or the learning algorithm}?
We offer an affirmative answer by presenting a line of work which we refer to as \textit{generalized input perturbation}.
% and present works on such type of \textit{generalized input perturbation}.

% input perturbation associated with the task or the modeling algorithm



\iffalse
version 2:
As an alternative, one can perform perturbation on \textit{representation space} and train a data generator to learn the distribution such that it is close to the input in representation space.
The DP guarantee arises from the Gaussian mechanism applied on the representation of the real data.
% private representation of the real data, obtained through the Gaussian mechanism.
The core challenge in instantiating the idea is to \textit{choose an appropriate representation}.
Catering to the distance metric Maximum Mean Discrepancy~(MMD)~\cite{gretton2012kernel} on probability measures, DP-MERF~\cite{harder2021dp} takes on the representation as random Fourier features appearing in the MMD approximation.
Informed by the uniqueness theorem of the characteristic function distance~(CFD)~\cite{sriperumbudur2011universality}, % which states the equivalence between zero CFD and identical data distribution
PEARL~\cite{liew2022pearl} chooses the characteristic function~(CF) representations.
The cost associated with the privacy embedding step is significantly lower than that on data space,
as a result of the low sensitivity of the kernel embedding space and the CF space.
To summarize, the chosen representations shall retain the desired properties for the data synthesis task and at the same time have low sensitivity.
% be suitable for the data synthesis task and have low sensitivity.
\fi

\iffalse
version 1:
DP-MERF~\cite{harder2021dp} takes on the representation as random Fourier features, while PEARL~\cite{liew2022pearl} chooses the characteristic function~(CF) representations as informed by the uniqueness theorem of the characteristic function distance~(CFD)~\cite{sriperumbudur2011universality}. 
PEARL further improves upon DP-MERF in the learning approach---Instead of using one fixed embedding as in DP-MERF, 
PEARL obtains multiple CFs and explicitly learns to re-weight them for the best representation through an adversarial objective.
In DP-MERF and PEARL, none of the steps other than the private embedding step induces any privacy cost.
The cost associated with the privacy embedding step is significantly lower than that on data space,
as a result of the low sensitivity of the kernel embedding space and the CF space.
\fi


% \fanr{provide a conclusion on what representation is appropriate;
% note the trade-off here: obtaining multiple representation increases privacy budget, yet enhances the learning performance (utility)
% }




% Generating synthetic data that are close to the noisy real data in the data space is known to have high cost~\cite{imtiaz2021synthetic}.
% An alternative is to 
% % DP-MERF~\cite{harder2021dp} and PEARL~\cite{liew2022pearl} thus 
% resort to the measure in the representation space---train data generators such that the synthetic data and the real data are close in distribution under a certain representation.
% % when measured in certain representations.
% The DP guarantee arises from the private representation of the real data, obtained through the Gaussian mechanism.
% % The DP guarantee comes as a result of deriving the private representation of the real data, by applying the Gaussian mechanism on the data representation.
% The core question in instantiating the algorithm is \textit{what representation is appropriate}.
% % Two critical questions in instantiating the algorithm are related to the selected representation and the learning approach.
% % They achieve the privacy guarantee through deriving the representations of the real data in a DP manner.
% % Concretely, 

\iffalse

DP-MERF~\cite{harder2021dp} takes on the representation as random Fourier features for one given kernel, 
and learns the data generator by minimizing the  Maximum Mean Discrepancy~(MMD)~\cite{gretton2012kernel} between the synthetic and real data in the representation space. %, a reproducing kernel Hilbert space.
PEARL~\cite{liew2022pearl} improves over DP-MERF on both the selected representation and the learning method.
It chooses the characteristic function~(CF) representations, 
as informed by the uniqueness theorem of the characteristic function distance~(CFD)~\cite{sriperumbudur2011universality}. % which states the equivalence between zero CFD and identical data distribution.
Instead of using one fixed embedding as in DP-MERF, 
PEARL obtains multiple CFs and explicitly learns to re-weight them for the best representation 
through an adversarial objective.
In DP-MERF and PEARL, none of the steps other than the private embedding step induces any privacy cost.
The cost associated with the privacy embedding step is significantly lower than that on data space,
as a result of the low sensitivity of the kernel embedding space and the CF space.

\fi

% The privacy embedding achieved by performing Gaussian mechanism 





% limitations of DP-MERF:
% representation not good enough, only one;
% learning through MMD formulation is more challenging


% DP-MERF, one fixed embedding, random fourier features for one given kernel
% learning limited by the fixed embedding;

% PEARL, multiple embeddings, can be reweighted; characteristic function
% 1. uniqueness theorem~\cite{sriperumbudur2011universality} of the CF, an ideal distance metric
% 2. adversarial formulation,  re-weighting

% private embedding: Gaussian mechanism on the derived embeddings



% learn a data generator such that *some* representation of the synthesized data is close to the real data.
% that representation of the real data is calculated in a private manner

% why not compare on original data space? --
% no need to do that (low-level representation good enough)
% [that is directly GAN (compare on data space)]
% learn a GAN that approximates the noisy input data
% derive noisy data is costly

% why the similarity on representation space is sufficient?



% intuition for input perturbation:
% can be used for any downstream processing and applications; too strong; 
% utility compromised a lot for specific downstream

% intuition for output perturbation:

% DP-MERF~\cite{harder2021dp}
% PEARL~\cite{liew2022pearl}

In DPGEN~\cite{chen2022dpgen}, input perturbation is guided by an unique approach of generative modeling.
The authors propose to generate images with the Langevin Markov chain Monte Carlo~(MCMC),
where an energy-based model~(EBM)~\cite{du2019implicit,lecun2006tutorial} is trained to learn the direction of movement in the MCMC.
Privatizing the direction of the input real data during pre-processing ensures DP on the generated image.
% Ensuring DP on the generated image is thus reduced to privatizing the movement direction for the input real data, achieved by a randomized response mechanism during pre-processing. 


\iffalse
Chen~\etal~\cite{chen2022dpgen} present a contrastingly different approach for data generation and design a privacy mechanism catering to this approach.
The proposed DPGEN learns to generate images with the Langevin Markov chain Monte Carlo~(MCMC),
where an energy-based model~(EBM)~\cite{du2019implicit,lecun2006tutorial} is trained to learn the direction of movement in the MCMC.
In this procedure, learning a private direction is sufficient for ensuring DP in the finally generated images, 
while privatizing the direction for real data can be done in the pre-processing stage via a randomized response mechanism.
\fanr{discussion on the empirical results}
\fi

\iffalse
Private post-GAN boosting~(PGB)~\cite{neunhoeffer2021private} boosts over the trained sequence of generators and discriminators in the post-processing stage, 
aiming to learn a distribution over the generated samples (produced by the generator sequence) to approximate the real data distribution, as discriminated by the mixture of the discriminator sequence.
DP is achieved through the update of the distribution on the generated samples via the private multiplicative weights method~\cite{hardt2010multiplicative}.
\fi

% These two works are typical examples where the pre-procesing or post-processing is guided by or dependent on the modeling efforts.

% via applying the  to update the .



% generate images with Langevin MCMC;
% train energy-based model to learn the `direction';
% randomize the direction in the training set;






\iffalse

Methods enforcing privacy mechanisms during pre-processing stage introduce DP noise to private data before training the generative model. The training process performed over the sanitized training set does not need to be private, since the privacy guarantee will be preserved according to the post-processing property of DP. An important advantage of this is that the number of training iterations is not constrained by the privacy budget.

\chulinr{Imtiaz~\etal~\cite{imtiaz2021synthetic} propose the first work to achieve DP} during pre-processing stage, which focuses on synthesizing smart health care data organized as tables. In their \textit{noisy input} setting, a GAN coupled with differential privacy mechanisms \chulin{@Zhuowen, why do they also need DP in the training stage? Also, not sure if we can say it is the "first" work according to its publication year} is trained after samples in the original dataset is transformed and sanitized with Laplacian noise.


Instead of perturbing original private data, more advanced methods~\cite{harder2021dp, liew2022pearl, torkzadehmahani2019dp} introduce noise to specific representations of private samples.
DP-MERF~\cite{harder2021dp} obtains a privacy-preserving generator by minimizing the Maximum Mean Discrepancy (MMD)\chulin{please cite} between perturbed true data and synthetic data. \chulin{please add one sentence to reason over why DP is guaranteed for the synthetic data }  To save computational cost on large-scale datasets, MMD is approximated using random Fourier features.
PEARL~\cite{liew2022pearl} privately embeds sensitive data with characteristic function (CF) and quantifies the discrepancy between real and generated data distributions with characteristic function distance, as in CF-based IPM-GANs~\cite{ansari2020characteristic}. \chulin{does the discrepancy mean to guarantee DP in this method? how?} It outperforms traditional training-stage methods DP-GAN~\cite{frigerio2019differentially} and DP-CGAN~\cite{torkzadehmahani2019dp}, which are based on DP-SGD\chulin{please cite}.



More recently, Chen~\etal~\cite{chen2022dpgen} propose DPGEN, an energy-guided network\chulin{cite or explain} for data generation via Langevin Markov chain Monte Carlo (MCMC) sampling method. The network is trained on sanitized data to indicate the direction of the true data distribution \chulin{so as to xxx improve utility?}. It abandons DPSGD which is commonly used for training differentially private deep models due to its drawbacks such as training inefficiency and large noise magnitude. DPGEN demonstrates {state-of-the-art} performance on high-dimensional image data (CelebA~\cite{liu2015faceattributes}) in terms of privacy-utility trade-off.

\noindent\textbf{Post-Processing Stage.}\quad

\fanm{@Zhuowen}:
\cite{neunhoeffer2021private} introduces a differentially private boosting algorithm that improves the quality of generated samples after the training of privacy-preserving generative model. Concretely, it considers samples produced by a sequence of generators obtained during GAN training and leverages the Private Multiplicative Weights~\cite{hardt2010multiplicative} method to optimize the generator. \chulin{please improve the description based on several questions: 1) What does the "privacy-preserving" mean in "the training of privacy-preserving generative model." Should the training stage satisfy DP? 2) a sequence of
generators  -- Is the sequence of models saved from different training epochs?  3)  how to optimize the generator with Private Multiplicative Weights? by enforcing consensus or something? 4) why optimizing the generator can improve utility? is there only one generator distilled from a sequence of generators in the end? 5) does the "Private Multiplicative Weights" method aim to satisfy DP in the post-processing stage? }

\fi
\vspace{-2mm} 
\subsubsection{Takeaways and Open Problems} \quad
We summarize the key takeaway in this subsection:
\begin{itemize}[leftmargin=*]
    \item \textbf{Generalized input perturbation is powerful.} \quad Well-designed generalized input perturbation frees practitioners from worrying about the privacy budget during model training
    and allows direct adaptation of the advanced model architectures and training algorithms.
    % Besides, {state-of-the-art} model architectures and training algorithms can be directly adapted since privacy is already guaranteed during pre-processing. 
    Consequently, advanced input perturbation methods have already demonstrated {state-of-the-art} performance.
\end{itemize}

% than \textit{state-of-the-art} privacy-preserving generative models via gradient perturbation and private knowledge aggregation and transfer.
We also identify an open problem for future research:
\begin{itemize}[leftmargin=*]
    \item \textbf{Suiting learning algorithms to noisy input.}\quad  The success of generalized input perturbation consists in designing task-specific algorithms for perturbing input data. Conversely, can we design specific learning algorithms that are more suited to the perturbed data? Since the noise injected for privacy purpose is more regularly distributed than in natural and adversarial settings, it is possible that some algorithms may lead to further improvement in the privacy-utility trade-off of deep generative models.
\end{itemize}

\fi



\iffalse

\subsection{Generation Stage Privacy Preservation}

\fan{may not need this part since it does not fit in our current framework}

DP-Image~\cite{liu2021dp},
DP imaging~\cite{li2021differentially},

PI-Net~\cite{chen2021perceptual},
DP facial obfuscation~\cite{croft2022differentially}

LDP~\cite{liu2021dp,li2021differentially,krishna2021adept},
\dx-privacy~\cite{chen2021perceptual,croft2022differentially} --- question: how do add noise in this privacy requirement?

comparison with the two privacy notions, if any

PCA~\cite{sakuma2021trajectory,croft2022differentially}


        The methods introduced in~\Cref{subsubsec:ae-formal-preprocess,subsubsec:ae-formal-train} are focused on DP guarantee.
        Moreover, most methods in~\Cref{subsubsec:ae-formal-train} intend to produce a DP generative model such that once the model is trained, it can be leveraged to generate infinite samples that satisfy DP guarantee.
        In this part, we are concerned with a stronger privacy definition that requires the indistinguishability for any two user.
        The main goal is not to obtain a DP generative model, but to obtain a sanitized dataset, where any two data records cannot be distinguished from each other from a privacy perspective~(\eg, identity).
        
        One naive approach to achieving the goal is to directly add noise to data records. However, the large noise scale would induce severe distortion to the data which leads to unfavorable utility.
        Given that the low-dimensional latent representation captures the salient information in the high-dimensional input,
        \textbf{latent manipulation}~\cite{krishna2021adept,sakuma2021trajectory,yang2022privacy,shamsabadi2022differentially,wen2022identitydp} has been proposed to achieve the goal of preserving data privacy while effectively retaining data utility.
        This approach first trains an AE that accomplishes the task of data reconstruction. 
        Next, the generation stage proceeds as follows: first introducing noise on the latent representation of the data sample, and then decoding the noisy latent back to the sample space.
        The noise added to the latent ensures the LDP property of the latent; due to the post-processing property of LDP, the decoded sample thus satisfies LDP as well.
        Specifically, to minimize the impact on data utility, when performing human face anonymization, 
        IdentityDP~\cite{wen2022identitydp} disentangle identity-related features from the identity-independent features and only perturb the former. 
        To save the privacy budget, Sakuma \etal~\cite{sakuma2021trajectory} further conducts a PCA transformation on the latent and adds noise to the transformed latent; 
        AdePT~\cite{krishna2021adept} adapts the training procedure by applying clipping accordingly so that the latent is encouraged to have small norm.
        Additionally, it is demonstrate that the synthesized dataset, when used to train a downstream ML model, can effectively defend against membership inference attacks~\cite{yang2022privacy,krishna2021adept}.


\subsubsection{Categorization and Paper Summary} 

\subsubsection{Takeaways and Open Problems}

\fi

% \subsection{Formal Privacy}
% \label{subsec:deep-formal}

% \subsubsection{Generation}~\\
% \label{subsubsec:deep-formal-gen}





% \subsubsection{Transformation}~\\







% \begin{table*}[htb]
% \small
% \caption{\small \textbf{Privacy-Preserving Distributed Generative Models based on GANs.} For aggregation methods, \textit{(Weighted) Average Aggregation} takes the (weighted) average of all user updates and \textit{Odds Value Aggregation} \cite{zhang2021training} mixes the updates in terms of odds value. \chulin{update the table with more papers}}
% \label{tab:gan-distributed-models}
% \resizebox{\linewidth}{!}{
% % \renewcommand{\arraystretch}{1.25}
% \begin{tabular}{llllllll}
% \toprule
% \textbf{Privacy Guarantee} & \textbf{Method} & \makecell[l]{\textbf{Models in} \\ \textbf{Server}} & \makecell[l]{\textbf{Models in} \\ \textbf{Client $i$}} & \makecell[l]{\textbf{Client $i$ to Server}\\\textbf{Communication}} & \makecell[l]{\textbf{Server to Client $i$}\\\textbf{Communication}} & \makecell[l]{\textbf{Aggregation}\\\textbf{Methods}} & \textbf{Utility Measures} \\
% \midrule

% \multirow{6}{*}{Access Control} 
% & FL-GAN \cite{hardy2019md} & $G$, $D$ & $G_i$, $D_i$ & $G_i$ and $D_i$ & $G$ and $D$ & Average & IS, FID \\
% & FedGAN \cite{rasouli2020fedgan} & $G$, $D$ & $G_i$, $D_i$ & $G_i$ and $D_i$ & $G$ and $D$ & Weighted Average & FID \\
% & MD-GAN \cite{hardy2019md} & $G$ & $D_i$ & gradients & generated images & Average & IS, FID \\ 
% & AsynDGAN \cite{chang2020multi} & $G$ & $D_i$ & gradients & generated images & Weighted Average & segmentation \\
% & TDGAN \cite{qu2020learn} & $G$ & $D_i$ & gradients & generated images & Weighted Average & segmentation \\
% & UA-GAN \cite{zhang2021training} & $G$ & $D_i$ & $D_i$ outputs, gradients & generated images & Odds Value & IS, FID, classification \\
% \bottomrule
% \toprule

% \multirow{2}{*}{Differential Privacy} 
% & DP-FedAvg-GAN \cite{augenstein2019generative} & $G$, $D$ & $D_i$ & gradients & $G$, $D$ & Average & debugging \\
% & GS-WGAN \cite{chen2020gs} & $G$ & $D_i$ & perturbed gradients & generated images & Average & IS, FID, classification \\
% \bottomrule
% \end{tabular}
% % \renewcommand{\arraystretch}{1}
% }
% \end{table*}




\iffalse

% the first version, considering studies with all kinds of privacy metrics


\section{The Guideline of Selecting PPDS algorithms}
\label{sec:guideline}
% \qb{@all, I'm trying to add a section to compare different PPGMs (e.g., statistical models vs GANs vs AEs in terms of scalability, efficiency, privacy, utility, etc) and give advice on the selection/deployment of PPGMs in real-world scenarios. Kindly let me know if you have any suggestions. Thank you!}

% \mirnegg{Thank you Qinbin! Actually we plan to add this part after addressing the comments in our own section. Currently we do not have anything concrete in mind, so it will be great if you could offer some suggestions.}

% \qb{@Yuzheng, I will finish a draft before 4/24 and then we can see how to improve it. I have some ideas in mind and I need to revisit existing studies to have a clearer picture.}

\qb{I have finished this draft section and it can be further improved after the improvement of previous sections. Kindly let me know if you have any suggestions. I have summarized the investigated studies in Table \ref{tab:model_summary} by data type and task. Please help to double check the table and see if there is anything wrong. Also, I have the following problems while writing the section.}

\qb{1. I find it challenging to compare different models in aspects of utility, efficiency, scalability, etc. Currently we only have experiments on GANs. I think the comparison between statistical models, GANs, and AEs would be very helpful. One possible solution is to theoretically/empirically compare the representative studies (e.g., Privbayes vs PATE-GAN vs DPGM as shown in Table \ref{tab:model_summary}).}

\qb{2. The organization of Section \ref{sec:stat},  \ref{sec:gan} and \ref{sec:ae} needs clarification/improvement. 1) In the aspect of data type, Section \ref{sec:gan} do not include studies on many types of data (e.g., graph). 2) Section \ref{sec:gan} introduces training GANs in the federated setting, which is not included in Section \ref{sec:stat} and Section \ref{sec:ae} (e.g., federated auto-encoder). 3) Section \ref{sec:ae} introduces many AE studies based on general privacy. General privacy actually does not provide any rigorous privacy guarantees. Then, what about general privacy in the other types of models? e.g., do PCA and GANs without DP satisfy general privacy? }

\qb{We can discuss and improve this section after the improvement of the previous sections.}




From Section \ref{sec:stat} to Section \ref{sec:ae}, we investigate and summarize existing studies on PPGMs by the type of models. Given the comprehensive solutions for PPGMs, one question is how to select the appropriate PPGMs in real-world scenarios. To provide a guideline for the selection of PPGMs, we summarize a practical selection process as shown in Figure \ref{fig:model_selection_process}. Specifically, we split the selection process into two steps: 1) selecting candidate models by \emph{hard factors} including the data type and task; 2) comparing the candidate models by \emph{soft factors} including the privacy guarantees and the utility. Next, we explain the above two steps in detail.

\subsection{Selecting Candidate Models by Hard Factors}
Given a real-world scenario for applying PPGMs, the data type and task are always fixed. As investigated in Section \ref{sec:stat} to Section \ref{sec:ae}, existing PPGMs cannot work for all kinds of data and some of them are designed for specific tasks (e.g., recommender system \citep{ren2019recommender,liu2019differentially}). Thus, the data type and task can be used to filter the PPGMs and get the candidate models as the first step. For the convenience of users, we summarize a scenario-oriented reference table (Table \ref{tab:model_summary}), which lists the investigated models by the data type and applicable task (or preserved property) of the synthetic data. Moreover, for each sublist of approaches, we identify the most recent paper that has received more than 20 citations according to Google Scholar as ``SOTA''. With Table \ref{tab:model_summary}, users can easily find the (SOTA) PPGMs that satisfy the required data type and task.

\qb{Let me know if you have any better definition of ``SOTA''.}

\input{tables/tab_ref}


\subsection{Comparing Candidate Models by Soft Factors}
Given the hard factors, there may be many existing PPGMs that satisfy the requirements. Thus, it is important to evaluate the candidate models and select the best. We identify privacy and utility as two key soft factors during the evaluation of PPGMs. Moreover, we suggest the following three steps as a standard evaluation pipeline.

\noindent \textbf{1) Determining the privacy metric.}\quad 
In reality, data regulations such as GDPR usually only protect the personal data and do not have restrictions on the usage of synthetic data. However, there are many attacks (e.g., membership inference attack \citep{membershipAttack}, attribute inference attack \citep{choi2017generating}) that can infer sensitive information about the personal data from the generated synthetic data. Thus, it is necessary to provide privacy guarantees for PPGMs. While there are many privacy metrics in the computer science community, we refer readers to \citep{wagner2018technical} for the comparison between different privacy metrics. However, in practice, given that DP has been a dominate privacy metric in PPGMs as shown in Table \ref{tab:model_summary}, we suggest DP as a default choice for privacy guarantees. After this step, we can further filter the candidate PPGMs and only evaluate the PPGMs that satisfy the selected privacy metric.

\noindent \textbf{2) Selecting the utility metric.}\quad 
If a specific task is given, we can directly evaluate and compare the performance of the candidate PPGMs on the tasks (e.g., classification error, RMSE). If we are selecting a PPGM for general purpose, besides evaluating the candidate PPGMs on some specific applications, we can also measure the data property preserved from the original dataset (e.g., inception score, $L_2$ distance). For the convenience of users, we have summarized the utility metrics for different kinds of data in Appendix \ref{adxsubsubsec:util-struc}.

\noindent \textbf{3) Evaluating the privacy-utility trade-off.}\quad 
There is always a trade-off between privacy and utility of PPGMs. For example, in differential privacy, a larger privacy budget usually implies a lower privacy level and higher utility. To fairly compare different PPGMs, we need to compare the privacy-utility curves (i.e., utility under different privacy levels) of them. Then, we can select the model with best utility satisfying a minimum privacy requirement or the model with highest privacy level satisfying a minimum utility requirement for deployment.

\subsection{A Case Study}
We conduct a case study to demonstrate how our guideline works in real-world scenarios. One scenario is that Google wants to improve its scene recognition service. It deploys many cameras in different areas to collect local data for training a scene recognition model. However, due to data regulations such as GDPR, the collected images cannot be transferred to a single server for training. Then, Google can apply PPGMs to generate and transfer synthetic data for training. Given the image data and the classification task, we can get the candidate models \citep{frigerio2019differentially,torkzadehmahani2019dp,chen2020gs,long2021gpate,wang2021datalens,chen2018differentially,edwards2016censoring,kim2019latent,kim2020selective} from Table \ref{tab:model_summary}. Since DP is the only possible rigorous privacy guarantee provided by the candidate models, Google may adopt DP as the privacy metric to enhance the privacy guarantee. Then, experiments on the models \citep{frigerio2019differentially,torkzadehmahani2019dp,chen2020gs,long2021gpate,wang2021datalens,chen2018differentially} are conducted to compare their utility-privacy trade-off. From our experiments on a scene recognition dataset (i.e., Place365) in Appendix \ref{app:benchmark}, DataLens\citep{wang2021datalens} can achieve the best utility under the same privacy level compared with the other available open-source PPGMs. Thus, DataLens may be the best choice for Google to generate synthetic data for training a scene recognition model.

% One scenario is that US Census wants to publish its collected statistics while protecting the personal data. Then, from Table \ref{tab:model_summary}, given the tabular data type and statistical queries as the task, 

\qb{I use this example since we have experiments on GANs. There are other applications such as medical data sharing and US Census that can be added in the future. Also, please feel free to share the real-world application you know with reference.}
\fi
% todo: new version, only comparing studies using DP





==> contents/5_selection.tex <==
\section{Selection Guidelines for PPDS algorithms}
\label{sec:guideline}
\fan{needs check; may drop}
% \qb{@all, I'm trying to add a section to compare different PPGMs (e.g., statistical models vs GANs vs AEs in terms of scalability, efficiency, privacy, utility, etc) and give advice on the selection/deployment of PPGMs in real-world scenarios. Kindly let me know if you have any suggestions. Thank you!}

% \mirnegg{Thank you Qinbin! Actually we plan to add this part after addressing the comments in our own section. Currently we do not have anything concrete in mind, so it will be great if you could offer some suggestions.}

% \qb{@Yuzheng, I will finish a draft before 4/24 and then we can see how to improve it. I have some ideas in mind and I need to revisit existing studies to have a clearer picture.}

From Section \ref{sec:stat} to Section \ref{sec:deep}, we investigate and categorize existing works on PPDS based on their methodologies, which provide \textit{researchers} with a systematic view of the field. On the other hand, given the massive amount of literature, one natural question from \textit{practitioners} is how to efficiently locate the  
desired algorithm in real-world scenarios. Here we provide guidelines for selection in the centralized setting, including a reference table of PPDS algorithms, 
%divided by data types and tasks, 
as well as some empirical principles summarized from existing studies.
\vspace{-4mm} 
\subsection{A Scenario-oriented Reference Table} %by Data Types and Tasks}
\vspace{-2mm} 
A real-world application of PPDS is mostly determined by the target data type and task. As such, these two factors can be used to
% Given a real-world scenario of PPDS, the data type and task are always fixed. Thus, they can be used to 
filter algorithms and obtain the candidate solutions as a first step for practitioners. %practice. For the convenience of practitioners, 
In light of this observation, we present a scenario-oriented reference table (\Cref{tab:model_summary}), which classifies
the papers that we cover in~\Cref{sec:stat} and \ref{sec:deep} by data types and applicable tasks.  %synthetic data. 
Moreover, for each sublist of approaches, 
we identify the paper that has received the highest number of citations according to Google Scholar as ``Most-cited'' and the latest paper as ``Fresh''. 
We also identify the methodologies used in the most-cited and fresh papers. With Table \ref{tab:model_summary}, practitioners can easily locate the set of possible candidates as well as the more competent ones within  
based on their need in real-world scenarios. Moreover, practitioners can refer to Table \ref{tab:stat} and Table \ref{tab:deep} for the detailed properties of these candidates with the help of Table \ref{tab:model_summary}.
% further pinpoint those with  
% potentially 
% based on their own 
% according to their data type and target task at hand. (SOTA) algorithms for PPDS that satisfy the required data type and task and test them. 
% From the table, we make the following observations.




\iffalse
\begin{itemize}[leftmargin=*]
    \item Tabular data 
     enjoy the most richest set of  as it is one of the most common data types in practice and has attracted researchers for a long history, while PPDS for text data are less explored and demand attention from researchers.
    \item Algorithms based on deep methods are usually capable of, while statistical methods are designed for 
    % Due to the high capability of deep learning models, deep methods based PPGMs are usually developed for general purpose, while many statistical methods based PPGMs are specially designed for a single task utilizing its statistical features. The latter usually provides provably utility guarantees.
\end{itemize}
\fi


\vspace{-2mm} 
\subsection{Empirical Principles}
\vspace{-2mm} 
In addition to the reference table, we also summarize some empirical principles based on our previous study to further facilitate the selection of PPDS algorithms.
% the evidence in existing 

 
% Based on the evidence in existing studies and competitions, we summarize the following empirical principles to further facilitate the selection of PPDS algorithms.

\begin{itemize}[leftmargin=*]
% \item For low-dimensional tabular data, statistical models are recommended due to their provably utility guarantee on specific tasks and empirically good performance, e.g., the marginal-based statistical methods \citep{mckenna2021winning, cai2021data} outperform the other methods from the results of NIST 2018 \citep{nist2018} and 2020 \citep{nist2020} contests.

\item Statistical methods are capable of capturing the intrinsic properties of structural data, and explicitly embody such understanding (of the properties) into the algorithm design, thus standing out in terms of the structured data synthesis. However, they usually fall short in generating unstructured data, as the signal within can hardly be captured and leveraged by statistical methods due to the restricted representation and learning power. 
%and therefore demands some brute-force (\eg, end-to-end learning).


\item {Powered by deep neural networks, deep methods can simultaneously handle a variety of data types without significant modifications, and is especially favorable for image synthesis.
%, can simultaneously handle a variety of data types with little modification. 
However, in terms of generating structured data, the quality is usually not as good as its counterpart as reflected by the NIST 2018 and 2020 contests, mainly due to the fact that the structural properties are not explicitly encoded in the architectural design or learning process.}

\item Deep methods serve as the silver bullet in the federated setting as the knowledge of each party can be aggregated through \textit{gradient averaging}. On the contrary, there is little study on applying statistical methods to federated synthesis, mainly because the information to be exchanged is unclear in the context of PPDS.
% statistical methods in the federated setting as it is challenging to design a proper way to aggregate statistical models.

% \item Some statistic method-based PPGMs may introduce unacceptable computation cost since the computational complexity is quadratic or even exponential in the number of attributes, including copula-based \citep{li2014differentially,asghar2019differentially,gambs2021growing} and query-based approaches \citep{hardt2012simple,vietri2020new,gaboardi2014dual}. Moreover, it is challenging for statistical models to capture the complex relation in the high-dimensional space due to their limited capacity. Privacy-preserving deep generative models are preferable for high-dimensional data.

% \item Practitioners are encouraged to measure the utility of candidate PPGMs by the performance on downstream applications or/and the data properties preserved from the original data. We have included a comprehensive list of utility metrics from existing studies in Appendix \ref{adxsubsubsec:util-struc} for reference. 
% , and tree-based approaches \citep{chen2012differentially,chen2012ngrams,he2015dpt,zhang2016privtree}.
\end{itemize}

% \qb{@all, please help to write any empirical rules you know for the selection/comparison among PPGMs.}




==> tables/tab_GAN.tex <==
% \begin{table*}[htb]
% \caption{\small \textbf{Privacy-Preserving graph Synthesis based on Deep Models}}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \toprule
% \multicolumn{3}{c}{\textbf{Privacy}} & \multicolumn{2}{c}{\textbf{Utility}} & \multicolumn{3}{c}{\textbf{Properties}} & \textbf{References} \\
% \cmidrule{1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htb]
\caption{\small \textbf{Privacy-Preserving graph Synthesis based on Deep Models} \fan{TODO: add explanations for the circle at each column; add cites for GAN, MA, RDP, etc.}}\label{tab:deep}
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllcccl}
\toprule
\multicolumn{3}{c}{\textbf{Privacy}} & \multicolumn{2}{c}{\textbf{Utility}} & \multicolumn{3}{c}{\textbf{Properties}} & \textbf{References} \\
\cmidrule{1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} 
Methodology & Privacy Guarantee & Privacy Accountant & Data Type & Model Type & \multicolumn{1}{l}{{Generality}} & \multicolumn{1}{l}{Scalability} & \multicolumn{1}{l}{\makecell[l]{Applicability \\  \quad \ in FL}} &  \\ \hline
\multirow{12}{*}{Gradient Perturbation} & \multirow{8}{*}{DP} & \multirow{5}{*}{MA} & \multirow{4}{*}{\makecell[l]{tabular / \\time series / \\network traffic}} & \makecell[l]{GAN, WGAN,\\ improved WGAN} & \CIRCLE & \Circle & \Circle & \cite{lu2017poster,fan2020relational,liu2019ppgan,xie2018differentially,frigerio2019differentially,fan2021dpnet} \\ \cline{5-9} 
 &  &  &  & AC-GAN & \CIRCLE & \Circle & \Circle & \cite{beaulieu2019privacy} \\ \cline{5-9} 
 &  &  &  & CTGAN & \Circle & \RIGHTcircle & \Circle & \cite{astolfi2021generating,wang2020part} \\ \cline{5-9} 
 &  &  &  & RCGAN & \Circle & \RIGHTcircle & \Circle & \cite{esteban2017real} \\ \cline{4-9} 
 &  &  & images & \makecell[l]{WGAN,\\improved WGAN} & \CIRCLE & \Circle & \Circle & \cite{xie2018differentially,zhang2018differentially,xu2019ganobfuscator,yang2020differential} \\ \cline{3-9} 
 &  & \multirow{3}{*}{RDP accountant} & \multirow{3}{*}{images} & WGAN & \CIRCLE & \RIGHTcircle & \Circle & \cite{schwabedal2020differentially,kossen2022toward} \\ \cline{5-9} 
 &  &  &  & improved WGAN & \CIRCLE & \RIGHTcircle & \RIGHTcircle & \cite{chen2020gs} \\ \cline{5-9} 
 &  &  &  & CGAN & \CIRCLE & \RIGHTcircle & \Circle & \cite{torkzadehmahani2019dp} \\ \cline{2-9} 
 & BDP & BDP accountant & images & improved WGAN & \CIRCLE & \RIGHTcircle & \Circle & \cite{triastcyn2020generating} \\ \cline{2-9} 
 & node-DP & standard composition & graph data & NetGAN & \Circle & \RIGHTcircle & \Circle & \cite{zhang2021differentially} \\ \cline{2-9} 
 & \multirow{2}{*}{edge-DP} & \multirow{2}{*}{MA} & \multirow{2}{*}{graph data} & NetGAN & \Circle & \RIGHTcircle & \Circle & \cite{zheng2021network} \\ \cline{5-9} 
 &  &  &  & GVAE, VAE-GAN & \Circle & \RIGHTcircle & \Circle & \cite{yang2020secure} \\ \hline
\multirow{3}{*}{\makecell[l]{Private Knowledge \\ Aggregation and Transfer}} & \multirow{3}{*}{DP} & MA & tabular & teacher-student, WGAN & \CIRCLE & \Circle & \RIGHTcircle & \cite{yoon2018pategan} \\ \cline{3-9} 
 &  & \multirow{2}{*}{RDP accountant} & tabular, images & teacher-student, DCGAN & \CIRCLE & \RIGHTcircle & \RIGHTcircle & \cite{long2021gpate} \\ \cline{4-9} 
 &  &  & images & teacher-student, DCGAN & \CIRCLE & \CIRCLE & \RIGHTcircle & \cite{wang2021datalens} \\ \hline
\multirow{2}{*}{Objective Perturbation} & \multirow{2}{*}{DP} & \multirow{2}{*}{N/A} & \multirow{2}{*}{images} & GAN & \CIRCLE & \Circle & \Circle & \cite{zhang2019differentially} \\ \cline{5-9} 
 &  &  &  & WGAN & \CIRCLE & \CIRCLE & \Circle & \cite{ma2020rdp} \\ \hline
\multirow{4}{*}{\makecell[l]{Generalized Input \\ Perturbation}} & \multirow{4}{*}{DP} & \multirow{4}{*}{N/A} & tabular & BGAN & \CIRCLE & \Circle & \Circle & \cite{imtiaz2021synthetic} \\ \cline{4-9} 
 &  &  & \multirow{3}{*}{images} & / & \CIRCLE & \RIGHTcircle & \Circle & \cite{harder2020differentially} \\ \cline{5-9} 
 &  &  &  & / & \CIRCLE & \CIRCLE & \Circle & \cite{liew2022pearl} \\ \cline{5-9} 
 &  &  &  & Langevin MCMC & \Circle & \CIRCLE & \Circle & \cite{chen2022dpgen} \\ \hline
\multirow{5}{*}{Federated Data Synthesis} & \multirow{3}{*}{DP} & \multirow{2}{*}{MA} & \multirow{2}{*}{images} & improved WGAN & \CIRCLE & \Circle & \CIRCLE & \cite{xin2022federated} \\ \cline{5-9} 
 &  &  &  & GAN & \CIRCLE & \Circle & \CIRCLE & \cite{zhang2021feddpgan} \\ \cline{3-9} 
 &  & on-average KL privacy & images & GAN & \CIRCLE & \Circle & \CIRCLE & \cite{triastcyn2020federated} \\ \cline{2-9} 
 & \multirow{2}{*}{user-level DP} & MA & images, text & GAN, RNN & \CIRCLE & \CIRCLE & \CIRCLE & \cite{augenstein2019generative} \\ \cline{3-9} 
 &  & RDP & images & improved WGAN & \CIRCLE & \CIRCLE & \CIRCLE & \cite{chen2020gs} \\
 \bottomrule
\end{tabular}%
}
\end{table*}

==> tables/tab_GAN_metric.tex <==
% \begin{table*}[htb]
% \caption{\small \textbf{Privacy-Preserving graph Synthesis based on Deep Models}}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllll}
% \toprule
% \multicolumn{3}{c}{\textbf{Privacy}} & \multicolumn{2}{c}{\textbf{Utility}} & \multicolumn{3}{c}{\textbf{Properties}} & \textbf{References} \\
% \cmidrule{1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htb]
\caption{\small \textbf{Privacy-Preserving graph Synthesis based on Deep Models} \fan{TODO: add explanations for the circle at each column; add cites for GAN, MA, RDP, etc.} DS-cls (seg) denotes downstream classification (segmentation). }\label{tab:deep}
\renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllccccl}
\toprule
\multicolumn{3}{c}{\textbf{Privacy}} & \multicolumn{2}{c}{\textbf{Utility}} &
\multicolumn{1}{c}{\textbf{Metric}} &\multicolumn{3}{c}{\textbf{Properties}} & \textbf{References} \\
\cmidrule{1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}  \cmidrule(lr){7-9} 
Methodology & Privacy Guarantee & Privacy Accountant & Data Type & Model Type  & & \multicolumn{1}{l}{{Generality}} & \multicolumn{1}{l}{Scalability} & \multicolumn{1}{l}{\makecell[l]{Applicability \\  \quad \ in FL}} &  \\ \hline
\multirow{12}{*}{Gradient Perturbation} & \multirow{8}{*}{DP} & \multirow{5}{*}{MA} & \multirow{4}{*}{\makecell[l]{tabular / \\time series / \\network traffic}} & \makecell[l]{GAN, WGAN,\\ improved WGAN} &   \makecell[l]{DS-cls, Bhattacharyya distance,  correlation \\  matrix, 
downstream clustering, query error,\\ distance to the closest record, hitting rate,\\
 performance agasint the inference attack}  & \CIRCLE & \Circle & \Circle & \cite{lu2017poster,fan2020relational,liu2019ppgan,xie2018differentially,frigerio2019differentially,fan2021dpnet} \\ \cline{5-10} 
 &  &  &  & AC-GAN & DS-cls & \CIRCLE & \Circle & \Circle & \cite{beaulieu2019privacy} \\ \cline{5-10} 
 &  &  &  & CTGAN & DS-cls, IS, distribution of specific attributes  & \Circle & \RIGHTcircle & \Circle & \cite{astolfi2021generating,wang2020part} \\ \cline{5-10} 
 &  &  &  & RCGAN &DS-cls& \Circle & \RIGHTcircle & \Circle & \cite{esteban2017real} \\ \cline{4-10} 
 &  &  & images & \makecell[l]{WGAN,\\improved WGAN} & \makecell[l]{DS-cls, IS, Jensen-Shannon scores, \\ performance against the inference attack } & \CIRCLE & \Circle & \Circle & \cite{xie2018differentially,zhang2018differentially,xu2019ganobfuscator,yang2020differential} \\ \cline{3-10} 
 &  & \multirow{3}{*}{RDP accountant} & \multirow{3}{*}{images} & WGAN & DS-seg, IS, FID& \CIRCLE & \RIGHTcircle & \Circle & \cite{schwabedal2020differentially,kossen2022toward} \\ \cline{5-10} 
 &  &  &  & improved WGAN & DS-cls, IS, FID & \CIRCLE & \RIGHTcircle & \RIGHTcircle & \cite{chen2020gs} \\ \cline{5-10} 
 &  &  &  & CGAN &DS-cls & \CIRCLE & \RIGHTcircle & \Circle & \cite{torkzadehmahani2019dp} \\ \cline{2-10} 
 & BDP & BDP accountant & images & improved WGAN & DS-cls, data debugging   & \CIRCLE & \RIGHTcircle & \Circle & \cite{triastcyn2020generating} \\ \cline{2-10} 
 & node-DP & standard composition & graph data & NetGAN &degree distribution& \Circle & \RIGHTcircle & \Circle & \cite{zhang2021differentially} \\ \cline{2-10} 
 & \multirow{2}{*}{edge-DP} & \multirow{2}{*}{MA} & \multirow{2}{*}{graph data} & NetGAN & downstream link prediction& \Circle & \RIGHTcircle & \Circle & \cite{zheng2021network} \\ \cline{5-10} 
 &  &  &  & GVAE, VAE-GAN & \makecell[l]{DS-cls, graph difference, degree distribution  } &  \Circle & \RIGHTcircle & \Circle & \cite{yang2020secure} \\ \hline
\multirow{3}{*}{\makecell[l]{Private Knowledge \\ Aggregation and Transfer}} & \multirow{3}{*}{DP} & MA & tabular & teacher-student, WGAN &  DS-cls & \CIRCLE & \Circle & \RIGHTcircle & \cite{yoon2018pategan} \\ \cline{3-10} 
 &  & \multirow{2}{*}{RDP accountant} & tabular, images & teacher-student, DCGAN & DS-cls, IS, FID & \CIRCLE & \RIGHTcircle & \RIGHTcircle & \cite{long2021gpate} \\ \cline{4-10} 
 &  &  & images & teacher-student, DCGAN & DS-cls&  \CIRCLE & \CIRCLE & \RIGHTcircle & \cite{wang2021datalens} \\ \hline
\multirow{2}{*}{Objective Perturbation} & \multirow{2}{*}{DP} & \multirow{2}{*}{N/A} & \multirow{2}{*}{images} & GAN &IS & \CIRCLE & \Circle & \Circle & \cite{zhang2019differentially} \\ \cline{5-10} 
 &  &  &  & WGAN &DS-cls & \CIRCLE & \CIRCLE & \Circle & \cite{ma2020rdp} \\ \hline
\multirow{4}{*}{\makecell[l]{Generalized Input \\ Perturbation}} & \multirow{4}{*}{DP} & \multirow{4}{*}{N/A} & tabular & BGAN & DS-cls & \CIRCLE & \Circle & \Circle & \cite{imtiaz2021synthetic} \\ \cline{4-10} 
 &  &  & \multirow{3}{*}{images} & / & DS-cls & \CIRCLE & \RIGHTcircle & \Circle & \cite{harder2020differentially} \\ \cline{5-10} 
 &  &  &  & / & DS-cls, FID, KID & \CIRCLE & \CIRCLE & \Circle & \cite{liew2022pearl} \\ \cline{5-10} 
 &  &  &  & Langevin MCMC & DS-cls, IS, FID & \Circle & \CIRCLE & \Circle & \cite{chen2022dpgen} \\ \hline
\multirow{5}{*}{Federated Data Synthesis} & \multirow{3}{*}{DP} & \multirow{2}{*}{MA} & \multirow{2}{*}{images} & improved WGAN & IS, FID, performance against model inverion attack &  \CIRCLE & \Circle & \CIRCLE & \cite{xin2022federated} \\ \cline{5-10} 
 &  &  &  & GAN & DS-cls & \CIRCLE & \Circle & \CIRCLE & \cite{zhang2021feddpgan} \\ \cline{3-10} 
 &  & on-average KL privacy & images & GAN & DS-cls& \CIRCLE & \Circle & \CIRCLE & \cite{triastcyn2020federated} \\ \cline{2-10} 
 & \multirow{2}{*}{user-level DP} & MA & images, text & GAN, RNN & data debugging  & \CIRCLE & \CIRCLE & \CIRCLE & \cite{augenstein2019generative} \\ \cline{3-10} 
 &  & RDP & images & improved WGAN & IS, FID, data debugging  & \CIRCLE & \CIRCLE & \CIRCLE & \cite{chen2020gs} \\
 \bottomrule
\end{tabular}%
}
\end{table*}

==> tables/tab_ae.tex <==
\begin{table*}[t]
\caption{\textbf{AE-based Methods for Privacy-preserving Generative Models.}
For privacy guarantee, we use GP and DP to denote general privacy and differential privacy.}\label{tab:ae}
\centering
\begin{tabular}
% { |p{1.8cm}|p{1cm}|p{1cm}|p{1cm}|p{2cm}|}
{lllll}
\toprule
\textbf{Methodology} & \textbf{Privacy Guarantee} & \multicolumn{2}{c}{\textbf{Data Type}} &  \textbf{References} \\ 
\midrule

\multirow{4}{*}{General AE} & 
\multirow{3}{*}{GP} & 
\multirow{1}{*}{Structured} & 
Tabular & 
\citep{maina2019subgroup,maina2019preservation,edwards2016censoring,louizos2016variational} \\
\cmidrule{3-5}
&&\multirow{2}{*}{Unstructured} & 
Image &
\citep{edwards2016censoring}\\
\cmidrule{4-5}
&&&Sensor & 
\citep{malekzadeh2018replacement,malekzadeh2019mobile}\\
\cmidrule{2-5}
&\multirow{1}{*}{DP} & 
\multicolumn{3}{c}{N/A}\\
\midrule

\multirow{3}{*}{Adversarial training} & 
\multirow{2}{*}{GP} & 
\multirow{2}{*}{Unstructured} & 
Image & 
\citep{kim2019latent,kim2020selective}\\
\cmidrule{4-5}
&&&Sensor & 
\citep{malekzadeh2019mobile,hajihassnai2021obscurenet}\\
\cmidrule{2-5}
&\multirow{1}{*}{DP} & 
\multicolumn{3}{c}{N/A}\\
% \midrule
\bottomrule
\toprule

\multirow{3}{*}{Direct adaptations of DP techniques} & 
\multirow{1}{*}{GP} & 
\multicolumn{3}{c}{N/A}\\
\cmidrule{2-5}
&\multirow{2}{*}{DP} & 
\multirow{2}{*}{Structured} & 
Tabular & 
\citep{ren2019recommender,phan2016differential,liu2019differentially}\\
\cmidrule{4-5}
&&& Graph &
\citep{yang2020secure}\\
\midrule

\multirow{3}{*}{Partition based techniques} & 
\multirow{1}{*}{GP} & 
\multicolumn{3}{c}{N/A}\\
\cmidrule{2-5}
&\multirow{2}{*}{DP} & 
\multirow{1}{*}{Structured} & 
Tabular & 
\citep{acs2018differentially,abay2018privacy}\\
\cmidrule{3-5}
&&\multirow{1}{*}{Unstructured} & 
Image &
\citep{chen2018differentially}\\
% \midrule
\bottomrule
\toprule

\multirow{2}{*}{GAN assisted methods} & 
\multirow{1}{*}{GP} & 
\multirow{1}{*}{Structured} & 
Tabular &
\citep{choi2017generating}\\
\cmidrule{2-5}
&\multirow{1}{*}{DP} & 
\multirow{1}{*}{Structured} & 
Tabular &
\citep{tantipongpipat2021differentially}\\
\midrule

\multirow{2}{*}{Latent representation manipulation} & 
\multirow{1}{*}{GP} & 
\multirow{1}{*}{Unstructured} & 
Sensor &
\citep{hajihassani2020latent,hajihassnai2021obscurenet}\\
\cmidrule{2-5}
&\multirow{1}{*}{DP} & 
\multirow{1}{*}{Unstructured} & 
Text &
\citep{krishna2021adept}\\
\bottomrule

\end{tabular}
\end{table*}

==> tables/tab_ae_2.tex <==
\begin{table*}[t]
\caption{\small \textbf{Privacy-Preserving Generative Models based on AEs.}
% For privacy guarantee, we use GP and DP to denote general privacy and differential privacy.
}\label{tab:ae-aligned}
\vspace{-3mm}
\centering
\resizebox{.99\linewidth}{!}{%
\begin{tabular}
% { |p{1.8cm}|p{1cm}|p{1cm}|p{1cm}|p{2cm}|}
{llllll}
\toprule
\textbf{Privacy Guarantee} &
\textbf{Methodology} &  
\multicolumn{2}{c}{\textbf{Data Type}} &  
\textbf{References} & 
\textbf{Utility Measures}\\ 
\midrule
\multirow{5}{*}{\makecell[c]{General\\Privacy}} & 
\multirow{2}{*}{General AE} & 
\multirow{1}{*}{Structured} & 
Tabular & 
\citep{maina2019subgroup,maina2019preservation,louizos2016variational} &
\makecell[l]{anomalous subgrup discovery, \\ misclassification rate}\\
\cmidrule{3-6}
&&\multirow{1}{*}{Unstructured} & 
Sensor & 
\citep{malekzadeh2018replacement,malekzadeh2019mobile} &
third-party applications, activity recognition\\
\cmidrule{2-6}

&\multirow{3}{*}{Adversarial training} & 
\multirow{1}{*}{Structured} & 
Tabular &
\citep{edwards2016censoring} & 
misclassification rate\\
\cmidrule{3-6}
&&\multirow{2}{*}{Unstructured} & 
Image & 
\citep{edwards2016censoring,kim2019latent,kim2020selective} & 
\makecell[l]{qualitative results, inception scores, misclassification rate}\\
\cmidrule{4-6}
&&&Sensor & 
\citep{malekzadeh2019mobile,hajihassnai2021obscurenet} &
activity recognition\\
\bottomrule
\toprule

\multirow{4}{*}{\makecell[l]{Differential\\Privacy}} & 
\multirow{2}{*}{Direct adaptations of DP techniques} & 
\multirow{2}{*}{Structured} & 
Tabular & 
\citep{ren2019recommender,liu2019differentially,phan2016differential} & 
RMSE, misclassification rate\\
\cmidrule{4-6}
&&& Graph &
\citep{yang2020secure} &
graph statistics, graph classification accuracy\\
\cmidrule{2-6}

& \multirow{2}{*}{Partition-based techniques} & 
\multirow{1}{*}{Structured} & 
Tabular & 
\citep{acs2018differentially,abay2018privacy} & 
clustering, SVM, K-Mgn\\
\cmidrule{3-6}
&&\multirow{1}{*}{Unstructured} & 
Image &
\citep{chen2018differentially} & 
misclassification rate\\
% \midrule
\bottomrule
\toprule

\multirow{3}{*}{\makecell[l]{Generall\\Privacy \& \\Differential\\Privacy}} &
\multirow{1}{*}{GAN assisted latent representation learning} & 
\multirow{1}{*}{Structured} & 
\multirow{1}{*}{Tabular} & 
\citep{choi2017generating} (GP), \citep{tantipongpipat2021differentially} (DP) & 
\makecell[l]{dimension-wise probability \& prediction, human \\expert, divergence, 1-Mgn, random forest}\\
\cmidrule{2-6}
&\multirow{2}{*}{Latent representation manipulation} & 
\multirow{2}{*}{Unstructured} & 
\multirow{1}{*}{Sensor} & 
\citep{hajihassani2020latent,hajihassnai2021obscurenet}~(GP) &
activity recognition, third-party applications\\
\cmidrule{4-6}
&&&\multirow{1}{*}{Text} & 
\citep{krishna2021adept}~(DP) &
intent classification\\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table*}

==> tables/tab_codelink.tex <==
\begin{table}[htp!]
    \centering
    \caption{Links to the publicly available repositories for the surveyed papers}\label{tab:codelink}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{ccl}
    \toprule
    \multirow{12}{*}{\makecell{Statistical \\models}} & \cite{hardt2012simple}     & \url{https://github.com/mrtzh/PrivateMultiplicativeWeights.jl}\\
    & \cite{gaboardi2014dual} & \url{https://github.com/ejgallego/dualquery} \\
    & \cite{vietri2020new} & \url{https://github.com/giusevtr/fem} \\
    & \cite{chanyaswad2019ron} & \url{https://github.com/inspire-group/RON-Gauss} \\
    & \cite{zhang2017privbayes} & \url{https://github.com/athenarc/PrivBayes}\\
    & \cite{mckenna2021winning} & \url{https://rb.gy/mlltjm} \\
    & \cite{cai2021data} & \url{https://github.com/caicre/PrivMRF} \\
    & \cite{zhang2021privsyn} & \url{https://github.com/agl-c/deid2_dpsyn} \\
    & \cite{li2014differentially} & \url{https://github.com/alxxrg/copula-shirley} \\
    & \cite{gambs2021growing} & \url{https://github.com/alxxrg/copula-shirley} \\
    & \cite{gursoy2018differentially} & \url{https://github.com/nomalocaris/DP-Star} \\
    & \cite{gursoy2018utility} & \url{https://github.com/git-disl/AdaTrace} \\
    
    \midrule
    \multirow{15}{*}{GAN} 
    & \cite{xie2018differentially} & \url{https://github.com/lancopku/DPGAN} \\
    & \cite{torkzadehmahani2019dp} & \url{https://github.com/reihaneh-torkzadehmahani/DP-CGAN} \\
      & \cite{harder2021dp} & \url{https://github.com/frhrdr/dp-merf} \\
      & \cite{liew2021pearl} & \url{https://github.com/lancopku/DPGAN} \\
      & \cite{chen2020gs} & \url{https://github.com/DingfanChen/GS-WGAN} \\
      & \cite{yoon2018pategan} &
      \makecell[l]{\href{https://github.com/vanderschaarlab/mlforhealthlabpub/tree/main/alg/pategan}{https://github.com/vanderschaarlab/mlforhealthlabpub/tree} \\ 
      \href{https://github.com/vanderschaarlab/mlforhealthlabpub/tree/main/alg/pategan}{/main/alg/pategan}} \\
      & \cite{long2019scalable} & \url{https://github.com/AI-secure/G-PATE} \\
      & \cite{wang2021datalens} & \url{https://github.com/AI-secure/DataLens} \\
    & \citep{hardy2019md} & \url{https://github.com/iDurugkar/GMAN} \\
    % & \citep{rasouli2020fedgan} & \url{} \\
    & \citep{chang2020multi} & \url{https://github.com/tommy-qichang/AsynDGAN} \\
    & \citep{qu2020learn} & \url{https://github.com/huiqu18/TDGAN-PyTorch} \\
    & \citep{zhang2021training} & \url{https://github.com/yz422/UAGAN} \\
    & \citep{augenstein2019generative} & \url{https://github.com/google-research/federated/tree/master/gans} \\
    & \citep{chen2020gs} & \url{https://github.com/DingfanChen/GS-WGAN} \\
    
    
    \midrule
    \multirow{8}{*}{AE} & \citep{yang2020secure}     &
    \makecell[l]{\href{https://github.com/haonan3/Secure-Network-Release-with-Link-Privacy}{https://github.com/haonan3/Secure-Network}\\
    \href{https://github.com/haonan3/Secure-Network-Release-with-Link-Privacy}{-Release-with-Link-Privacy}}\\
    & \citep{choi2017generating} & \url{https://github.com/mp2893/medgan} \\
    & \citep{tantipongpipat2021differentially} & \url{https://github.com/DPautoGAN/DPautoGAN} \\
    & \citep{kim2019latent} & \url{https://github.com/tgisaturday/PPAP} \\
    & \citep{kim2020selective} & \url{https://github.com/tgisaturday/PPSGAN}\\
    & \citep{malekzadeh2018replacement} & \url{https://github.com/mmalekzadeh/replacement-autoencoder} \\
    & \citep{malekzadeh2019mobile} & \url{https://github.com/mmalekzadeh/motion-sense} \\
    & \citep{hajihassnai2021obscurenet} & \url{https://github.com/sustainable-computing/ObscureNet} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:stat}
\end{table}

==> tables/tab_ref.tex <==
\begin{table*}[]
\caption{\textbf{A reference table for the selection of candidate PPGMs. ``SM'' denotes statistical model.}}
% 4/22
\label{tab:model_summary}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{Data Type}                       & \textbf{Applicable Task}%/Preserved Property& \textbf{Privacy Guarantee}                                       
& \textbf{Model}               & \textbf{Approaches} & \textbf{SOTA} \\ \midrule
\multirow{11}{*}{Tabular data}   & \multirow{5}{*}{Task-independent}               & \multirow{3}{*}{DP}                                                           & SM                  &   \citep{chanyaswad2019ron,chen2015differentially,mckenna2021winning,cai2021data,zhang2017privbayes,li2014differentially,asghar2019differentially,gambs2021growing}         &Privbayes\citep{zhang2017privbayes}      \\ \cmidrule{4-6} 
                            &                                                 &                                                                               & GAN                 &\citep{xie2018differentially,yoon2018pategan,long2021gpate}            & PATE-GAN\citep{yoon2018pategan}     \\ \cmidrule{4-6} 
                            &                                                 &                                                                               & AE                  &\citep{acs2018differentially,abay2018privacy,chen2018differentially,tantipongpipat2021differentially}            &  DPGM\citep{acs2018differentially}    \\ \cmidrule{3-6} 
                            &                                                 & Plausible Deniability                                                         & SM                  &\citep{bindschaedler2017plausible}            &PD\citep{bindschaedler2017plausible}      \\ \cmidrule{3-6} 
                            &                                                 & General Privacy                                                                  & AE                  &\citep{choi2017generating,louizos2016variational,edwards2016censoring,maina2019subgroup,maina2019preservation}            &medGAN\citep{choi2017generating}      \\ \cmidrule{2-6} 
                            & Statistical queries                             & DP                                                                            & SM                  &\citep{hardt2012simple,vietri2020new,gaboardi2014dual,li2011compressive}            &FEM\citep{vietri2020new}      \\ \cmidrule{2-6} 
                            & Covariance matrix & DP                                                                            & SM                  &\citep{zhou2009differential,blocki2012johnson}            &JL\citep{blocki2012johnson}      \\ \cmidrule{2-6} 
                            & Sparse regression & Information Resistance                                                                           & SM                  &\citep{zhou2009compressed}            &SR\citep{zhou2009compressed}      \\ \cmidrule{2-6} 
                            & Distance between records                          & DP                                                                            & SM                  &\citep{kenthapadi2012privacy,xu2017dppro}            &Dppro\citep{xu2017dppro}      \\ \cmidrule{2-6} 
                            & Recommender system                              & DP                                                                            & AE &\citep{ren2019recommender,liu2019differentially}            &---    \\ \cmidrule{2-6}
                            & Human behavior prediction                       & DP                                                                            &AE                     & \citep{phan2016differential}           &dPAH\citep{phan2016differential}  \\ \bottomrule\toprule
\multirow{3}{*}{Trajectory data} & \multirow{3}{*}{Task-independent}               & DP                                                                            & SM &  \citep{chen2012differentially,chen2012ngrams,he2015dpt,zhang2016privtree,mir2013dp,roy2016practical,gursoy2018differentially,gursoy2018utility,gursoy2020utility,shao2013publishing}          &DP-Star\citep{gursoy2018differentially}      \\ \cmidrule{3-6} 
                            &                                                 & Plausible Deniability                                                         &SM                     &\citep{bindschaedler2016synthesizing}            &PPLT\citep{bindschaedler2016synthesizing}      \\ \cmidrule{3-6} 
                            &                                                 & $k^{\tau,\epsilon}$-Anonymity &SM                     & \citep{gramaglia2017preserving}           &k-merge\citep{gramaglia2017preserving}      \\ \bottomrule\toprule
\multirow{4}{*}{Graph}      & \multirow{2}{*}{Task-independent}               & \multirow{2}{*}{DP}                                                           & SM                  &\citep{mir2012differentially,sala2011sharing,wang2013preserving,lu2014exponential,xiao2014differentially,jorgensen2016publishing,chen2020publishing,proserpio2012workflow,chen2014correlated,zhu2019dp,nguyen2016network,nguyen2015differentially}            &AGMDP\citep{jorgensen2016publishing}      \\ \cmidrule{4-6} 
                            &                                                 &                                                                               & AE                  &\citep{yang2020secure}            &---      \\ \cmidrule{2-6} 
                            & Clustering                                      & DP                                                                            & SM                  &\citep{mulle2015privacy}            &PIG\citep{mulle2015privacy}      \\ \cmidrule{2-6} 
                            & Cut-queries                                     & DP                                                                            & SM                  & \citep{blocki2012johnson}           &JL\citep{blocki2012johnson}      \\ \bottomrule\toprule
\multirow{4}{*}{Image}      & \multirow{3}{*}{Task-independent}               & \multirow{2}{*}{DP}                                                           & GAN                 &\citep{frigerio2019differentially,torkzadehmahani2019dp,chen2020gs,long2021gpate,wang2021datalens}            &GS-WGAN\citep{chen2020gs}      \\ \cmidrule{4-6} 
                            &                                                 &                                                                               & AE                  & \citep{chen2018differentially}           &DP-GM\citep{chen2018differentially}      \\ \cmidrule{3-6} 
                            &                                                 & General Privacy                                                                 & AE                  &\citep{edwards2016censoring,kim2019latent}            &ALFR\citep{edwards2016censoring}      \\ \cmidrule{2-6} 
                            & Classification                                  & General Privacy                                                                 & AE                  &\citep{kim2020selective}            &---      \\ \bottomrule\toprule
Text                        & Task-independent                                & DP                                                                            & AE                  &\citep{krishna2021adept}            &---      \\ \bottomrule\toprule
\multirow{2}{*}{Sensor}     & Task-independent                                & General Privacy                                                                          & AE                  &\citep{malekzadeh2018replacement}            &Replacement AE\citep{malekzadeh2018replacement}      \\ \cmidrule{2-6} 
                            & Activity Recognition                            & General Privacy                                                                 & AE                  &\citep{malekzadeh2019mobile,hajihassani2020latent,hajihassnai2021obscurenet}            &AAE\citep{malekzadeh2019mobile}      \\ \bottomrule
\end{tabular}
}
\end{table*}

